A Thorough Investigation of Content-Defined Chunking Algorithms for Data Deduplication

Data deduplication emerged as a powerful solution for reducing storage and bandwidth costs in cloud settings by eliminating redundancies at the level of chunks. This has spurred the development of numerous Content-Defined Chunking (CDC) algorithms over the past two decades. Despite advancements, the current state-of-the-art remains obscure, as a thorough and impartial analysis and comparison is lacking. We conduct a rigorous theoretical analysis and impartial experimental comparison of several leading CDC algorithms. Using four realistic datasets, we evaluate these algorithms against four key metrics: throughput, deduplication ratio, average chunk size, and chunk-size variance. Our analyses, in many instances, extend the findings of their original publications by reporting new results and putting existing ones into context. Moreover, we highlight limitations that have previously gone unnoticed. Our findings provide valuable insights that inform the selection and optimization of CDC algorithms for practical applications in data deduplication.

==> Dockerfile <==
#FROM ubuntu:latest

#RUN apt update
#RUN apt install -y texlive-latex-recommended texlive-fonts-recommended texlive-latex-extra texlive-publishers texlive-science texlive-fonts-extra
FROM texlive/texlive:latest

#RUN tlmgr update --self --all

#RUN apt update
#RUN apt

WORKDIR /paper-builder
COPY . .

RUN latexmk -C
RUN latexmk -bibtex -interaction=nonstopmode

RUN bash -c 'echo "\pdfoutput=1" | cat - main.tex > main2.tex'
RUN mv main2.tex main.tex
#RUN sed -i -e '1i \pdfoutput=1' master.tex
RUN python3 arxiv_collector.py -p biblatex -p acmart --latexmk-deps .deps main.tex




==> algorithms/quickcdc.tex <==
\caption{$\textproc{QuickCDC}(d, l)$}
\hspace*{\algorithmicindent} \textbf{Input:} Data stream $d$, data length $l$ \\
\hspace*{\algorithmicindent} \textbf{Predefined:} Front length $n$, end length $m$, minimum chunk length $\lambda_\text{min}$
\begin{algorithmic}[1]
	\State $\text{Front} \gets d[i;i+n]$
	\State $\lambda_F \gets H_F[Front]$
	\If{$\lambda_F \neq$ null}
  		\State $\text{End} \gets d[i+\lambda_F-m;i+\lambda_F]$
		\State $\lambda_E \gets H_E[End]$
		\If{$\lambda_F = \lambda_E$}
			\State \Return $i+\lambda_E$
		\EndIf
	\EndIf
	
	\For{$i \leftarrow i+\lambda_\text{min}$ to $l$}
		\State Run inner algorithm, add chunk to cache.
	\EndFor
\end{algorithmic}

==> fig/csd_rabin_dataset_faceted_4096_v1.tex <==
% Created by tikzDevice version 0.12.4 on 2023-12-19 11:53:00
% !TEX encoding = UTF-8 Unicode


==> fig/csd_rabin_dataset_faceted_4096_v2.tex <==
% Created by tikzDevice version 0.12.4 on 2023-12-19 11:53:00
% !TEX encoding = UTF-8 Unicode


==> fig/csd_rabin_random_4096_v1.tex <==
% Created by tikzDevice version 0.12.4 on 2023-12-19 11:53:00
% !TEX encoding = UTF-8 Unicode


==> fig/csd_rabin_random_4096_v2.tex <==
% Created by tikzDevice version 0.12.4 on 2023-12-19 11:53:00
% !TEX encoding = UTF-8 Unicode


==> fig/csd_rabin_random_target_faceted_v1.tex <==
% Created by tikzDevice version 0.12.4 on 2023-12-19 11:53:00
% !TEX encoding = UTF-8 Unicode


==> fig/csd_rabin_random_target_faceted_v2.tex <==
% Created by tikzDevice version 0.12.4 on 2023-12-19 11:53:00
% !TEX encoding = UTF-8 Unicode


==> sections/algorithms/quickcdc.tex <==
As we noted in \cref{sec:background},
Rabin-based chunking has often been critiqued for its high chunk-size variance
and low throughput.
Hence, over the years, the class of BSW algorithms has experienced many innovations.
QuickCDC is one of the algorithms currently at the edge of these developments.
QuickCDC is a combination of multiple techniques 
that have been proposed in previous work \cite{ddelta,fastcdc,rapidcdc}
plus additional optimizations,
both of which we will explain in the following.

Generally, QuickCDC can be decomposed into three layers.
It is noteworthy that the original authors of QuickCDC did not perform this decomposition,
but we find it helpful for illustrative purposes.
The layers can be described as follows:
\begin{enumerate*}
	\item The innermost layer, which runs a chunking algorithm of choice.
	\item A leaping layer, which skips a minimum chunk size before running the \ac{BSW} algorithm.
	\item A caching layer, which we refer to as a \emph{driver}.
	This caches information about previously emitted chunks and, upon encountering a likely duplicate, skips \ac{BSW} processing entirely and emits the block as-is.
\end{enumerate*}

In the original publication, the authors use \textit{normalized} Gear as the innermost algorithm,
as it is fast and postpones the chunk size distribution to after the minimum chunk size.
However, the choice of chunking algorithm is not strictly limited.

The leaping layer skips a configurable minimum chunk size before initializing and running the inner algorithm.
This may negatively impact content dependence (\cf \cref{sec:background:csVariance}).
With an appropriately high degree of normalized chunking, however,
it can be relatively safe to skip over a minimum chunk size,
because the algorithm has a very low probability of producing a chunk with a small size anyway.
Ultimately, this technique just further aids in improving throughput.

Finally, the caching driver is the real innovation in QuickCDC.
It is used to cache previously emitted blocks,
enabling the system to skip processing subsequent duplicates entirely.
The mechanism employs feature vectors $v_F, v_E$ of sizes $n$ and $m$ bytes respectively, for the front and end of a block.
The cache consists of a table $H$ of $(v_F,v_E,l)$ tuples, with $l$ being the size of the cached chunk.
We show an example of this in \cref{tab:quickcdc}, with $n=m=3$.
After a chunk is emitted, \ie, whenever a new chunk is begun, the first $n$ bytes of the input data are compared against the cache table.
If a matching $v_F$ is found, the end of the potential duplicate chunk, determined by $l$, is checked to see if the last $m$ bytes also match $v_E$. 
If both the front and end feature vectors match, a chunk of size $l$ is emitted without invoking the inner chunking algorithm.
This mechanism is visualized in \cref{fig:quickcdc}.

Notably, the original publication does not specify the exact data structures to be used for the cache.
Obvious choices are hash maps or arrays indexed \via $v_F$, for lookups in $\mathcal{O}(1)$.
Furthermore, it is possible to decompose the table into two, one holding $(v_F,l)$ tuples and the other $(v_E,l)$ tuples.
Additionally, the mechanisms for cache eviction are not specified.
It would be possible to extend the mechanism in a way to hold a \emph{list} of potential blocks starting with $v_F$,
by, \eg, indexing \via $(v_F,l)$ tuples instead, or simply storing lists of $(v_E, l)$ tuples for each $v_F$.
We leave these explorations for future work.
%\leo{Double check if the original paper needs decomposition into $H_F$ and $H_E$.
%We don't want to implement a different algorithm.
%If yes: Update example table. If no: update algorithm}
%\marcel{our pseudocode corresponds to their pseudocode, and also our example table corresponds to a table. I don't think it's wrong, this table, $H_F$, and $H_E$, just represent different indices from the same data}

\begin{table}[ht]
    \centering
    \caption{Example of the map table in QuickCDC.}
	\input{tables/quickcdc.tex}
    \label{tab:quickcdc}
\end{table}

\begin{figure}
    \centering
    \input{figures/quickcdc.tex}
    \caption{QuickCDC Caching mechanism.}
    \label{fig:quickcdc}
\end{figure}

\begin{algorithm}
	\input{algorithms/quickcdc.tex}
	\label{alg:quickcdc}
\end{algorithm}




==> sections/appendices/ae_stochastics.tex <==
\begin{definition}
	In AE, $i+h$ marks a cut-point if it is the first position for which $B_i\geq\max\{B_j\}_{j=i+1}^{i+h}$.
\end{definition}

In order for any byte $B_i$ at position $i$ to become subject to the matching condition,
all previous bytes $B_{j<i}$ must have failed the matching condition $B_j\geq\max\{B_k\}_{k=j+1}^{j+h}$.
However, these are not independent events.
The event $B_{i-1}<\max\{B_{j}\}_{j=i}^{i+h-1}$ influences the expectation of $B_{i},\ldots,B_{i+h}$, and therefore affects the probability $B_i<\max\{B_j\}_{j=i+1}^{i+h}$.
So does every previous condition back to $B_{i-h-1}<\max\{B_j\}_{j=i-h}^i$ as it still influences the expected value of $B_i$.
This leads to a \textbf{chain of recursive conditional probabilities} that we express as:

\begin{equation}
\begin{split}
    \mathrm{P}(i+h\text{ marks cut-point})= \mathrm{P}(B_i\geq \max\{B_j\}_{j=i+1}^{i+h}\mid B_{i-1}<\max\{B_j\}_{j=i}^{i+h-1}\land\ldots\land
    B_{i-h-1}<\max\{B_j\}_{j=i-h}^{i})\cdot\\\ldots\cdot\mathrm{P}(B_2<\max\{B_j\}_{j=3}^{h+2}\mid B_1<\max\{B_j\}_{j=2}^{h+1})\cdot\mathrm{P}(B_1<\max\{B_j\}_{j=2}^{h+1})
\end{split}
\end{equation}

For the purpose of readability, we introduce the abbreviation $M_h := \max\{B_i\}_{i=1}^h$ to denote the maximum value among $h$ bytes. 
As we are assuming uniformly distributed random data, and bytes are discrete variables in $[0,255]$,
the probability for any byte $X$ to take any value $0\leq x\leq 255$ is $P(X=x)=1/256$.
Furthermore, $P(X<x)=\frac{x}{256}$, $P(X\geq x)=\frac{256-x}{256}$, $P(X<Y)=\frac{1}{2}$, and $P(X\leq Y)=\frac{257}{512}$.

\begin{lemma}
	The cumulative distribution function $F_M(m)=\mathrm{P}(\max\{B_i\}_{i=1}^h\leq m)$ follows
	\begin{equation}
		F_{M_h}(m)=\mathrm{P}(B_1\leq m\land\ldots B_h\leq m)=\left(\frac{m+1}{256}\right)^h\quad\text{for }0\leq m\leq 255
	\end{equation}
	
	and can be used to express the probability mass function of $M_h$:

	\begin{equation}
    	\mathrm{P}(M_h = m) = F_{M_h}(m)-F_{M_h}(m-1)=\left(\frac{m+1}{256}\right)^h-\left(\frac{m}{256}\right)^h\quad\text{for }0\leq m\leq 255
    \label{eq:ae_mh_m}
	\end{equation}

	Further, a lower bound $x$ changes this distribution to

	\begin{equation}
    	\mathrm{P}(M_h=m\mid M_h\geq x) = \left(\frac{m-x+1}{256-x}\right)^h-\left(\frac{m-x}{256-x}\right)^h\quad \text{for } 0 \leq m \leq 255 \quad \text{and} \quad 0 \leq x \leq 255.
	\label{eq:eight}
	\end{equation}
\end{lemma}

\begin{figure}[h]
    \centering
    \input{figures/ae_pmf.tex}
    \caption{Probability mass function for $M_h$. Note, $m$ is discrete; line plots were chosen for readability. As $h$ increases, the expected value for $M_h$ converges to 255.}
    \label{fig:ae_pmf}
\end{figure}

Intuitively, low values for $M_h$ become asymptotically the larger $h$, as more bytes are contributing to the maximum value. We illustrate this in \cref{fig:ae_pmf}. 
Further, $\lim_{h\to\infty} E(M_h) = 255$.
For instance, with $h=2000$, $\mathrm{P}(M_h=255)>0.999$.
\cf~\eqref{eq:eight}).
That is, $\mathrm{P}(M_h=m\mid M_h\geq x)\geq\mathrm{P}(M_h=m)$ for any $0\leq x\leq 255$.

The practical implication of this is that when AE is used with target chunk sizes beyond \qty{2}{KB},
the approximation that $M_h\approx 255$ can be used to simplify the problem to

\begin{equation}
    \mathrm{P}(i+h\text{ is cut-point}) = \mathrm{P}(B_i=255) = \frac{1}{256}.
\end{equation}

On average, therefore, a chunk cut-point will be found after the evaluation of 256 bytes.
Hence, target chunk size for AE is $\mu\approx h+256$ for large values of $h$;
the parameterization is determined by $h\approx\mu-256$.
We continue with extended calculations for small target chunk sizes.

The probability for a random byte to fail the matching condition is

\begin{equation}
    \mathrm{P}(X < \max\{B_i\}_{i=1}^{h}) = \sum_{m=0}^{255} \mathrm{P}(X < m)\cdot\mathrm{P}(\max\{B_i\}_{i=1}^{h}=m).
\end{equation}


The probability in this form would apply to the first byte of the sequence, \ie, it is equivalent to $\mathrm{P}(B_1<\max\{B_i\}_{i=2}^{h+2})$.

The second byte $B_2$, which only gets evaluated under the pre-condition that $B_1<\max\{B_i\}_{i=2}^{h+1}$, faces the same condition as its precursor, but has a different probability as it is conditioned:

\begin{equation}
\begin{split}
    \mathrm{P}(B_2<\max\{B_i\}_{i=3}^{h+2}\mid B_1<\max\{B_i\}_{i=2}^{h+1})\\
    =\sum_{x=0}^{255} \mathrm{P}(B_2=x\mid B_1<\max\{B_i\}_{i=2}^{h+1})\cdot\mathrm{P}(x<\max\{B_i\}_{i=3}^{h+2}\mid B_1<\max\{B_i\}_{i=2}^{h+1})\\
    =\sum_{x=0}^{255} \Bigg( \mathrm{P}(B_2=x\mid B_1<\max\{B_i\}_{i=2}^{h+1}) \cdot
 \sum_{m=x+1}^{255} \mathrm{P}(\max\{B_i\}_{i=3}^{h+2}=m\mid B_1<\max\{B_i\}_{i=2}^{h+1}) \Bigg)
\end{split}
\label{eq:seven}
\end{equation}

The expectation of $B_2$ and the expectation of $\max\{B_i\}_{i=3}^{h+2}$ are shifted towards higher values, given that $B_1<\max\{B_i\}_{i=2}^{h+1}$.

The two conditional probabilities needed to solve \eqref{eq:seven} are less trivial. 
We are deriving $\mathrm{P}(B_2=x\mid B_1<\max\{B_i\}_{i=2}^{h+1})$ using Bayes' formula, which transforms the expression to

\begin{equation}
    \mathrm{P}(B_2=x\mid B_1<\max\{B_i\}_{i=2}^{h+1}) = \frac{\mathrm{P}(B_1<\max\{B_i\}_{i=2}^{h+1}\mid B_2=x)\cdot\mathrm{P}(B_2=x)}{\mathrm{P}(B_1<\max\{B_i\}_{i=2}^{h+1})}.
\end{equation}

We derive the inversed conditional probability $\mathrm{P}(B_1<\max\{B_i\}_{i=2}^{h+1}\mid B_2=x)$ in the following lemma.

\begin{lemma}
The probability of a byte $B_1$ being smaller than the maximum value among the $h$ bytes in its horizon, given that one of the bytes $B_2$ is known, can be expressed as

	\begin{equation}
	\begin{split}
    	\mathrm{P}(B_1 < \max\{B_i\}_{i=2}^{h+1})\mid B_2=x)=
	    \mathrm{P}(x\geq \max\{B_i\}_{i=3}^{h+1})\cdot\mathrm{P}(B_1<x) \;\oplus\;\\ 
 	   \mathrm{P}(\max\{B_i\}_{i=3}^{h+1}>x)\cdot\mathrm{P}(B_1<\max\{B_i\}_{i=3}^{h+1})\mid \max\{B_i\}_{i=3}^{h+1}>x)
	\end{split}
	\end{equation}
	\label{lemma:ae_prob1}
\end{lemma}

\begin{proof}
	Given $B_2=x$, we know that $\max\{B_i\}_{i=2}^{h+1}\geq x$. That is, either $x$ is the maximum in this horizon and $x\geq \max\{B_i\}_{i=3}^{h+1}$, or the remaining bytes are and $\max\{B_i\}_{i=3}^{h+1}>x$. 
\end{proof}

\begin{lemma}
	The probability distribution for the maximum value among $h$ bytes, given that the preceding byte is smaller than the maximum value in its horizon, 
	can be expressed as 
	\begin{equation}
	\begin{split}
    	\mathrm{P}(\max\{B_i\}_{i=3}^{h+2}=m\mid B_1<\max\{B_i\}_{i=2}^{h+1})
	    =(h-1)\cdot \mathrm{P}(B_3=m \land B_j\leq m\;\forall j\in[4,h+1] \mid B_1<\max\{B_i\}_{i=2}^{h+1}) \cdot \\ 
	    \mathrm{P}(B_{h+3}\leq m)+
    	\mathrm{P}(B_{h+3}=m)\cdot\mathrm{P}(B_3\leq m\mid B_1<\max\{B_i\}_{i=2}^{h+1})^{h-1}
	\end{split}
	\end{equation}
	\label{lemma:ae_prob}
\end{lemma}

\begin{proof}
%	We are describing the probability of any one byte $B_j\in \{B_i\}_{i=3}^{h+2}$ having the value $m$
%while all the remaining bytes $B_{k\neq j} \leq m$ in the horizon $k\in[3,h+2]$.
The expectation about a subset of bytes $\{B_i\}_{i=3}^{h+2} \cap \{B_i\}_{i=2}^{h+1} = \{B_i\}_{i=3}^{h+1}$ is influenced by the given condition,
\ie, all bytes in the target sequence except for its final byte $B_{h+2}$.
Intuitively, one byte will be $m$ while the remaining $h-1$ bytes of the intersecting horizon are $\leq m$.
By multiplying the chance for one of these bytes by $h-2$, we account for every byte in the intersecting horizon to be in place of the maximum value. 
In the formula, we used $B_3$ as an arbitrary placeholder, as any byte in the affected sequence yields identical chances.
Simultaneously, we also verify that the final (non-intersecting) byte $B_{h+3}\leq m$.
Finally, we account for the case that the final byte $B_{h+3}=m$ and all bytes in the conditioned sequence $\leq m$.
\end{proof}

We further derive the following probability in support of \cref{lemma:ae_prob}:
\begin{equation}
\begin{split}
  \mathrm{P}(B_3=m \land B_j\leq m\;\forall j\in[4,h+1] \mid B_1<\max\{B_i\}_{i=2}^{h+1}) \\ 
   	 = \mathrm{P}(B_3=m\mid B_1<\max\{B_i\}_{i=2}^{h+1})\cdot\mathrm{P}(B_4\leq m\mid B_1<\max\{B_i\}_{i=2}^{h+1})^{h-2}
\end{split}
\label{eq:ten}
\end{equation}

The evaluation of the expression in \eqref{eq:seven} using \cref{lemma:ae_prob1,lemma:ae_prob} 
accumulates six hierarchies of sum-loops. 
The complexity further depends on the size of $h$.
However, even with low values for $h$, 
the evaluation of the expression turned out to be computationally too expensive (we interrupted the execution after two hours).
Therefore, we deem exact analytical solutions impracticable.
We recommend an experimental approach for tuning $h$ for low target chunk sizes,
and making use of the approximation $h\approx\mu-256$ for target chunk sizes beyond \qty{2}{KB}.

==> sections/appendices/pci_stochastics.tex <==
\begin{definition}
	In PCI, $i+w-1$ marks a cut-point if it is the first position for which $\sum_{j=i}^{i+w}\text{popcount}(B_j) \geq \theta$.
\end{definition}

The probability for a sequence of $w$ randomly distributed bytes $B_1,\ldots,B_w$ to accumulate a specific popcount $p$ is described as

\begin{equation}
	\mathrm{P}\left(\sum_{i=1}^w\text{popcount}(B_i)=p\right) = \frac{\binom{8w}{p}}{2^{8w}}.
\end{equation}

Therefore, we can trivially determine that for this byte sequence to match PCI's matching condition, the probability equals

\begin{equation}
	\mathrm{P}\left(\sum_{i=1}^w\text{popcount}(B_i)\geq\theta\right) = \sum_{p=\theta}^{2^{8w}} \frac{\binom{8w}{p}}{2^{8w}}.
	\label{eq:pci_p_first}
\end{equation}

For position $i+w$ to set a chunk boundary, all positions $j+w$ where $j<i$ must have subsequently failed the matching condition.

In \eqref{eq:pci_p_first}, we contemplate the probability for the first possible position in the byte sequence to mark a chunk boundary.
The next possible position (\ie, $1+w$) is contingent upon the preceding position failing to satisfy the matching condition. 
Additionally, the expectation regarding the popcount within its window is also influenced by this event.

Intuitively, $1+w$ sets a new chunk boundary only if the insufficiency of 1-bits in the preceding window is compensated for by the 1-bits introduced by the new byte, with the 1-bits of the leftmost byte that dropped out being deducted.
Formally, this is the event of $\text{popcount}(B_{w+1})-\text{popcount}(B_1) > \theta-\sum_{i=1}^w\text{popcount}(B_i)$.
This event occurs when the popcount in $B_1$ is $a\in[0,7]$,
the popcount in $B_2,\ldots,B_w$ is $m=[\theta-8, \theta-8+a]$,
and the popcount in $B_{w+1}$ is $z=[m, 8]$.
This probability is encapsulated in the following equation:

\begin{equation}
	\mathrm{P}\left(\sum_{i=2}^{w+1}\text{popcount}(B_i)\geq\theta \mid \sum_{i=1}^w\text{popcount}(B_i)<\theta\right) =
	\sum_{a=0}^7\left( \frac{\binom{8}{a}}{2^8} \cdot \sum_{m=a+1}^8 \left( \frac{\binom{w-8}{m}}{2^{w-8}} \cdot \sum_{z=m}^8 \frac{\binom{8}{z}}{2^8} \right) \right)
\end{equation}

As with AE and RAM (\cf \cref{app:ae_probs,app:ram_probs}),
the consideration for later chunk boundaries, \ie, $i=3,4,\ldots$, only increases the complexity of this equation as the events become recursively dependent on one another.
Because of the high complexity of this probability and the unavailability of an approximation, we recommend determining parameters in PCI empirically.

==> sections/appendices/ram_stochastics.tex <==
\begin{definition}
	In RAM, $h+i$ marks a cut-point if it is the first position for which $B_i\geq\max\{B_{j>h}\}_{j=1}^{h}$.
\end{definition}

The case for RAM is more trivial than it is for AE.
As the maximum value $M_h=\max\{B_j\}_{j=0}$ is fixed, the expectation is not dependent on consecutive events. 

Based on the probability distribution about the maximum value among $h$ bytes we derived in \eqref{eq:ae_mh_m}, 
we can obtain its expected value through

\begin{equation}
	E(M_h)=\sum_{m=0}^{255} m\cdot\mathrm{P}(M_h=m).
\end{equation}

Here again, $\lim_{h\to\infty} E(M_h) = 255$.

The analysis of the relationship between $h$ and $\mu$ in RAM now breaks down to finding how many random bytes $X$ it takes \textit{on average} for one to be greater than or equal $M_h$:

\begin{equation}
\begin{aligned}
	&& x\cdot\mathrm{P}(X\geq E(M_h)) &= 1\\
	\Leftrightarrow && \qquad x&=\frac{1}{\mathrm{P}(X\geq E(M_h))}
\end{aligned}
\end{equation}

As $h$ acts as an inherent minimum chunk size, $\mu=h+x$, and therefore

\begin{equation}
	\mu = h + \frac{1}{\mathrm{P}(X\geq E(M_h))}.
\end{equation}

After insertion, we conclude the following formula in order to determine the target chunk size:

\begin{equation}
\begin{split}
	\mu &= h + \left(\frac{256
	-\sum_{m=0}^{255}m\cdot\left(\left(\frac{m+1}{256}\right)^h-\left(\frac{m}{256}\right)^h\right)}{256}\right)^{-1} \\
	&= h + \left(1-\frac{1}{256}\sum_{m=0}^{255}m\cdot\left(\left(\frac{m+1}{256}\right)^h-\left(\frac{m}{256}\right)^h\right)\right)^{-1} \\
	%	\mu &= h + \left(\frac{1}{256}-\frac{1}{256}\cdot\sum_{m=0}^{255} m \cdot \left( \left( \frac{m+1}{256} \right)^h - \left( \frac{m}{256} \right)^h \right) \right)^{-1} \\
%	\mu &= h + \left(256 - 256 \cdot \sum_{m=0}^{255} m \cdot \left( \left( \frac{m+1}{256} \right)^h - \left( \frac{m}{256} \right)^h \right) \right)^{-1} \\
%	\mu &= -h+ \frac{256}{\left(\frac{1}{256}\right)^h (256-\sum_{m=1}^{256} m\cdot((m+1)^h-m^h)}
\end{split}
\end{equation}

Because of its complex transcendental nature, we must solve $h$ numerically.

In addition to that, we can provide the same approximation for target chunk sizes beyond \qty{2}{KB} that we concluded in \cref{app:ae_probs}.
As $\lim_{h\to\infty}E(M_h)=255$, and $\mathrm{X\geq 255}=\frac{1}{256}$, we can akin to AE use the approximation $\mu\approx h+256$ for $h>$ \qty{2}{KB}.




==> sections/background/boundary-shift-problem.tex <==
As introduced earlier, \ac{FSC} represents the most primitive but also most efficient chunking method.
In \ac{FSC}, a chunk cut-point is set after every $k$ bytes.
However, this method suffers from the boundary-shift problem~\cite{lbfs,ae,tian2017does},
which describes the detrimental effect of any local modification on global deduplication.
By locality, we refer to the position within a file. 
This could already be, for instance, the addition or removal of a comma in a text file.
In \cref{fig:boundaryShiftProblem}, we illustrate this exact problem.
While the corresponding chunk boundaries of File A shift,
the effective chunk boundaries do not.

\begin{figure}
	\centering
	\include{figures/boundary-shift-problem.tex}
  \vspace{-2em}
  \caption{Boundary-shift problem.}
  \label{fig:boundaryShiftProblem}
\end{figure}

Let $F = \{c_1, \ldots, c_n\}$ be the set of chunks for a file split using FSC,
and let $F'$ denote the set of chunks for the same file after some modification.
The abstract goal of effective deduplication is to represent both files with as little space as needed, \ie, such that $|F \cup F'|$ is minimal.
Ideally, the symmetric difference $F \triangle F'$ should therefore only contain the chunks 
whose bytes are directly affected by the modification.
For FSC, however, if the modification alters the size of the file, \ie,
the amount of added bytes is unequal to the amount of deleted bytes,
it will cause \emph{all} subsequent chunk cut-points to shift.
This means that even a tiny modification inside $c_i$ is likely 
to alter all chunks $c_{j \geq i} \in F'$,
disregarding potentially long sequences of redundant content.
On average, and assuming a modification to occur at any random position within a file, $i = |F|/2$.

In a system where \emph{local} modifications are frequent, \eg,
files are versioned or otherwise correlated,
this potential loss in deduplication for redundant content is critical.
Note that this is mostly the case with \emph{text-based} files,
such as source code, plain text documents, or PDF files.
On the other hand, executables and compressed archive formats such as ZIP or RAR present a high degree of non-locality:
Their contents are packed tightly, in a way where small changes to the source file can cause arbitrarily large changes in the output file.
Many multimedia file formats,
such as image, audio, and video,
also utilize internal compression.
We refer to those files as \emph{binary} files.
In datasets where binary files are predominant,
perceived correlation between the files will not necessarily reflect correlation on the byte-level,
and modification to a file therefore is not \enquote{local}.
Thus, the boundary-shift problem is only concerned with low-entropy/text-based files.


==> sections/background/chunk-size.tex <==
Algorithms have to run over files to determine their chunk boundaries,
individual chunks need to be indexed,
and metadata needs to be generated.
Those processes are costly in terms of computation, 
and with regard to metadata also to memory and disk space.
When it comes to indexing,
this effect is amplified with smaller chunk sizes,
as they result in a greater number of chunks
for which fingerprints must be calculated.
While smaller chunks generally provide more opportunities for deduplication,
they also escalate metadata storage demands.
With this consideration,
Wallace et al.~\cite{wallace2012characteristics}
determine the theoretical optimum at around \qty{8}{\kilo\byte}.
It depends, however, on the nature of the data,
specifically the frequency and length of redundant sequences.
The chunk size should be brought in accordance with
the expected length of redundant sequences,
and also the space in between those sequences,
such that those sequences can be isolated.
In practical applications, 
where processing speed often becomes a determining factor
(\eg, Windows Server~\cite{winServer2012,msftDedup}, ZFS~\cite{zfs}, GPFS~\cite{gpfs}, and~\cite{ceph}),
chunk sizes typically range between 32 and \qty{256}{\kilo\byte}.
%\leo{is that 32 B or 32 KiB?}
%\marcel{kb}
When using a \ac{CDC} algorithm, the process of finding chunking boundaries is usually the biggest drag on efficiency.
However, the efficiency of the chunking process itself is, in most cases, not affected by the chunk size.
\ac{CDC} algorithms generally execute the same set of machine instructions on every byte,
regardless of the chunking decision.
Minimum chunk size skipping or high-level strategies (\cf \cref{sec:background:rechunking})
might, however, indeed exert an influence on the computational speed in relation to the chunk size.

==> sections/background/incremental-sync.tex <==
Incremental synchronization, as for example in rsync~\cite{rsync}, presents a special application of \ac{CDC}.
It does not consider data reduction in storage systems, but the incremental synchronization of data between machines.
Files are chunked on both ends to determine the segments of data that need to be transmitted.
However, the produced chunks are never stored.
This condition puts a relaxation on the constraint for low chunk-size variance.
In 2019, Zhang \etal proposed \ac{MII}, and one year later \ac{PCI}, as algorithms specialized to this application.

%In the incremental data synchronization scenario, the focus is on minimizing.
%%In recent years, some algorithms that specialize in incremental data synchronization have emerged.
%Chunking for data synchronization has its focus on minimizing bandwidth requirements.
%Deduplication efficacy is therefore prioritized over computational efficiency and also chunk-size variance.
%
%
%
%In more recent years, another set of algorithms has emerged
%that specifically targets data synchronization (\cf rsync~\cite{rsync}),
%and explicitly prioritizes chunk \emph{stability} over chunk-size variance.
%Chunk stability refers to the resistance to byte shifting in a modified version of a previous file, \ie,
%the modification should affect the least amount of chunks.
%Variance in chunk size are disregarded in this class of algorithms
%since the resulting chunks are not intended for storage purposes.
%
%\ac{MII}~\cite{mii}
%was proposed as an algorithm specifically designed for this use case.
%The algorithm defines a chunk boundary after each position $i$
%where $B_i>B_{i-1}>\ldots>B_{i-w}$ for a small $w$.
%This is expected to achieve very good resistance to byte shifting,
%because the chunk boundary only relies on a small sequence of $w$ bytes to remain stable.
%On their datasets of incremental data, the authors concluded a 13--34\,\%
%gain in deduplication ratio compared to other CDC algorithms.
%The chunk-size variance is similar to that of Rabin-based CDC, \ie, poor.
%Additionally, it demonstrates suboptimal performance when handling low-entropy strings.
%However, as mentioned above,
%both of these are not a priority for the use case of data synchronization.
%Furthermore, the authors claim that, since the MII algorithm is computationally much more efficient than traditional Rabin-based CDC,
%it achieves throughput comparable to AE.
%
%The same authors later proposed \ac{PCI}~\cite{pci},
%which similarly cuts files based on short data intervals.
%\ac{PCI} checks the number of 1-bits in a window, \ie, the \emph{popcount},
%and compares it to a preset threshold value to determine chunk boundaries.
%This provides better control of the expected chunk size than MII.
%The new algorithm promises better chunk size stability
%and outperformed MII in terms of deduplication performance,
%at the cost of throughput.


==> sections/background/leap-based.tex <==
%% FastCDC and Leap-based
As FastCDC has shown, leap-based techniques
can significantly improve throughput in the BSW algorithm.
Already prior to FastCDC, this potential has been recognized by other researchers. 
Yu et al. \cite{leapBased} proposed a technique (we refer to it as \textit{LeapCDC})
that is based on the idea of leaping to avoid unnecessary computations.
To this end, they rely on weak conditions that, if not fulfilled, allow the algorithm to leap forward.
Even though LeapCDC reached a noticeable performance increase compared to Rabin-based CDC,
it still underperforms BSW with modern rolling hash functions like Gear,
hence also FastCDC.

%% RapidCDC
RapidCDC~\cite{rapidcdc} makes further improvements to the efficiency of FastCDC
by introducing the notion of duplicate locality,
and furthermore, the \emph{locality-quantification sequence (LQ-sequence)}.
The authors observed that changes to a file are often unevenly distributed (\ie, local).
This creates contiguous sequences of deduplicable chunks.
They propose to extend the metadata that is used to describe a file
with the size of the subsequent chunk attached to every chunk's fingerprint.
That is, a file's metadata consists of a sequence of pairs \textit{<chunk fingerprint, size of next chunk>}, the LQ-sequence.
When processing a file and recognizing the recent chunk's fingerprint in the file system,
RapidCDC looks up the size of the following chunk
in the LQ-sequence of those files containing the current chunk's fingerprint.
Based on the assumption that the likelihood of the same sequence repeating itself in the current file is high,
the sliding window jumps to the suggested position,
skipping the search for a chunk boundary.
The assumption can then be verified by comparing the fingerprint of the potential new chunk.
Using this more aggressive leap-based strategy,
RapidCDC claims up to $33\times$ better efficiency than regular CDC.
However, this obviously depends on the dataset and its deduplicability.
Contrary to FastCDC, RapidCDC does not implement normalized chunking.
However, it employs a minimum chunk size.

%% QuickCDC
Recently, a new algorithm, QuickCDC~\cite{quickcdc}, was proposed
to optimizes the approach of RapidCDC,
claiming $11\times$ its throughput and even a slightly improved deduplication ratio.
QuickCDC maintains a global table of the first $n$ and last $m$ bytes of each chunk, and its size.
Using this, the implementation can,
upon finding a known start sequence at the beginning of a new chunk,
check whether the last $m$ bytes at the expected end position match,
and emit the chunk without fingerprinting.
Furthermore, QuickCDC employs the normalized chunking method introduced in FastCDC.
This presumably explains the slightly elevated deduplication ratio.

% Jump-based 2023
Finally, the most recent algorithm on our list is Jump-based Chunking (JC)~\cite{jin2023accelerating}.
JC is based around \ac{BSW} algorithms and introduces a new condition for \enquote{speculative} jumping to speed up chunking.
The idea of jumping is inspired by LeapCDC.
However, while LeapCDC only skips positions that are definitely no cut-points,
JC jumps more often by taking speculative risks.
To this end, JC introduces two masks:
the mask that determines a cut-point,
and a mask that determines when the algorithm should jump a specific length.
The cut-point mask is embedded into the mask for jumping.
That is, when a fingerprint matches with the cut-point mask, it always also matches the jump-point mask.
The cut-point mask will have at least one 1-bit more in its mask,
making its evaluation less probable than the jump-point mask's.
In their experiments on real-world datasets,
JC maintained deduplication efficacy to state-of-the-art CDC algorithms such as Gear or AE,
while achieving $2\times$ higher throughput.


==> sections/background/normalized-chunking.tex <==
%% Regression chunking and FastCDC}
Chunking algorithm developers have addressed the issue of high chunk-size variance in various ways.
In 2012, El-Shimi et al.~\cite{el2012primary} proposed a \textit{regression chunking} mechanism
that loosens the matching condition as the chunk grows;
essentially shrinking $b$, thereby gradually increasing the probability of the matching condition.
Tian et al.~\cite{tian2017does} discovered the frequent occurrence of consecutive maximum-sized chunks in real-world datasets.
%This is likely due to longer segments of low entropy in files.
%They address this issue by proposing \textit{Elastic Chunking},
%which adjusts the matching condition during the chunking process 
%once it observes too many consecutive maximum-sized chunks,
%and resets it back once this issue is fixed.
In 2016, FastCDC~\cite{fastcdc} extends the idea of regression chunking to \ac{NC},
wherein the authors implement a stringent matching condition 
while the current index remains below the target chunk size, 
subsequently relaxing this condition once the index surpasses the target.
This makes pathological chunk sizes on both sides asymptotically unlikely,
while also maintaining content-dependence.
We find the same principle also applied in \cite{hirsch2020dynamic}.
It further allows the algorithm in FastCDC
to \enquote{safely} skip the defined minimum size in each chunk
(without missing out on too many potential cut-points),
and thereby gain a substantial speed-up.
The idea is conceptually demonstrated in \cref{fig:normalizedChunking}.
By exploring different parameters for the matching condition before and after the target chunk size,
FastCDC aims to mimic a normalized distribution.
However, in reality, the algorithm is expected to produce one logarithmic decay starting at the chunk size minimum,
and another one every time the matching condition is relaxed.
Since the matching condition is relaxed starting from the target chunk size, 
this is also where the distribution reaches its peak.
The name \enquote{normalized chunking} is therefore misleading;
we will still use it throughout the paper to refer to this method.

%We explain this algorithm in further detail in \cref{sec:algorithms:bsw} 
%and present the achieved distributions, based on our own experiments, in \cref{sec:distribution}.
%Together with other optimizations,
%FastCDC claims $10\times$ the throughput of Rabin-based CDC
%while maintaining similar deduplication ratio.
%The latter is surprising because skipping and the employment of an inconsistent matching condition
%would be associated with missed opportunities for better chunking boundaries.
%Another way to think about it is to imagine increasing levels of NC as a gradual approach toward FSC.
%The authors achieve the highest deduplication ratio with NC-2; higher even than without any deployment of NC
%(however, with minimum chunk size skipping).
%In our experiments, shown in \cref{sec:dedup}, we investigate the effects of NC.
%
\begin{figure}
\centering
\scalebox{0.8}{\input{plots/chunk-size-normal.tex}}
\caption{Conceptual diagram of normalized chunking as proposed in FastCDC (target: \qty{8}{KB}; min: \qty{4}{KB}; max: \qty{12}{KB}).}
\label{fig:normalizedChunking}
\end{figure}


==> sections/background/parallelization.tex <==
Many researchers over the years have improved upon the algorithmic efficiency of existing CDC algorithms.
Since most computers nowadays run multi-core processors,
a lot of effort in the last decade has been put into the investigation
of the utility of parallelization in order to further enhance throughput of existing CDC algorithms.
This is not a trivial task since CDC algorithms are inherently sequential,
since every chunk boundary depends on the preceding chunk boundary.
The goal of parallelization is thus to increase throughput while maintaining \emph{chunking invariability}.
This ensures 
that the parallelized execution of CDC on a file 
returns the same set of chunks as the sequential execution of CDC on the same file would.
This condition is highly desirable as it otherwise affects content-dependency.
Furthermore, care must be taken when evaluating increases in throughput, as the entire deduplication process can become I/O bound at some point.

%% Pipelining
However, there are still parts in the entire process of data deduplication which can be parallelized safely.
Determining the chunk boundaries within a file is merely the first
in a four-stage sequential process:
%
\begin{enumerate}[itemsep=0ex,partopsep=1ex,parsep=1ex,label=\textbf{S\arabic*.},leftmargin=1cm]
	\item \label{item:chunking} Chunking
	\item \label{item:fp} Hashing for fingerprinting
	\item \label{item:indexing} Indexing
	\item \label{item:metadata} Writing file metadata and chunk data
\end{enumerate}
%
These steps can be run independently for each new chunk,
thus enabling pipelined parallelism.
In other words, one can compute the hash for the first chunk,
while the CDC algorithm is busy determining the second chunk.
This idea is schematically visualized in~\cref{fig:pipeline}.
Note also that some of the steps are CPU-demanding (\ref{item:chunking} \& \ref{item:fp}),
while others depend on memory and/or disk reading and writing capacity (\ref{item:indexing} \& \ref{item:metadata}).
This is interesting because it allows 
to not only make the most of having multiple CPUs,
but also different hardware components now working at the same time.
Note further that this strategy is applicable to data deduplication using \emph{any} chunking algorithm.
The technique of pipelining has been a part in the design of 
high-performing storage deduplication system architectures,
such as in P-Dedupe~\cite{pdedupe} and the system proposed in~\cite{guo2011building}.

\begin{figure}[htbp]
  \centering
  \include{figures/parallel-chunking-pipeline.tex}
  \vspace{-2em}
  \caption{Parallel processing of the pipeline that creates a chunk after each new chunk boundary determination.}
  \label{fig:pipeline}
\end{figure}

P-Dedupe described a second strategy to further exploit parallelization
in the process of chunk boundary determination itself (\ref{item:chunking})
by leveraging the multicore nature of modern CPUs.
To this end, the authors describe a ``divide, conquer, and connect'' approach,
which refers to the concept of chunking multiple segments of a file (using BSW) in parallelized threads,
and then re-chunking a small part 
at the end and the beginning of two adjacent segments, respectively.
It only requires rechunking of the string 
$(A_{n-w},\ldots,A_n,B_1,\ldots,B_{w-1})$,
where $A$ is the last and $B$ is the first chunk of two adjacent section
and $w$ refers to the size of the sliding window
to ensure chunking invariability.
The authors claim near-linear speedup.

%\begin{figure}[htbp]
%  \centering
%  \include{figures/parallel-segments.tex}
%  \vspace{-2em}
%  \caption{Concurrent chunking of segments of a file on multiple threads.}
%  \label{fig:parallelSegments}
%\end{figure}

\ac{MUCH}~\cite{much} is another algorithm that enables parallel CDC with chunking invariability.
In contrast to the approach described in P-Dedupe, 
it is not bound to BSW as its underlying algorithm,
but instead is agnostic to the CDC algorithm in use.
The procedure in \ac{MUCH} is based on a method the authors call \textit{Dual Mode Chunking},
which is applied on each segment.
It consists of a \textit{slow} mode and an \textit{accelerated} mode.
The difference is that, during slow mode,
the chunking algorithm will not enforce minimum and maximum chunk sizes.
In each file segment, chunking starts in slow mode, 
and switches to accelerated mode as soon as it encounters the marker chunk $c_m$.
The \textit{marker chunk} is defined as the first chunk
(or second if $m=1$)
to fulfill the following condition:
%
\begin{equation}\label{eq:markerChunk}
	\lambda_\text{min} \leq \,|c_m|\, \leq \lambda_\text{max} - \lambda_\text{min}
\end{equation}
%
Where $\lambda_\text{min}$ and $\lambda_\text{max}$ denote the thresholds of minimum and maximum chunk length, respectively.
All subsequent chunks will be chunked in the accelerated mode until the end of the segment is reached.
After all threads have finished, 
the next step is to merge the resulting chunks produced for the segments in all threads
without the final and complete sequence of chunks for the file
to violate chunking invariability.
The authors call this step \textit{chunk marshalling}.
To this end, for two adjacent segments $A$ and $B$,
we require the last produced chunk in $A$, let that be $a_n$,
and the first chunks in $B$ up until the marker chunk
(\ie, $b_1,\ldots,b_m$).
Let us refer to this range of chunks as $X=(a_n,b_1,\ldots,b_m)$.
This sequence is likely to have boundaries corrupted through the method of parallelized chunking,
and furthermore, chunk sizes that are not compliant with the minimum and maximum chunk size setting.
Both issues are targeted in the process of chunk marshalling,
which in its basics works by the following substeps:
%
\begin{enumerate}
	\item \textbf{Chunk Coalescing:} 
For each $c_i\in X$,
coalesce $c_i$ with $c_{i+1}$ 
if $|c_i| < \lambda_\text{min}$.
	\item \textbf{Chunk Splitting:} 
For each $c_i\in X$,
split $c_i$ into $(c_{i_1}, c_{i_2})$
with $|c_{i_1}| = \lambda_\text{max}$
if $|c_i| > \lambda_\text{max}$.
\end{enumerate}
%
Mind that during chunk coalescing, 
when $c_i$ and $c_{i+1}$ are getting coalesced, 
the algorithm continues at $c_{i+2}$.
Similarly, when $c_i$ is split into $(c_{i_1}, c_{i_2})$, 
the same procedure will recursively be applied to $c_{i_2}$.
Because of the predicate set on the marker chunk
(\cf \cref{eq:markerChunk}),
the chunk marshalling is guaranteed to result in chunks 
compliant to the minimum and maximum chunk size restrictions.
Finally, this method will also result in a coherent sequence of chunks
that comply with chunking invariability.

In an experimental analysis,
the authors of \ac{MUCH} were able to conclude that their methodology is able 
to reach a performance benefit that scales linearly with the number of CPU cores.

Similar to \ac{MUCH}, although different in its technical details,
operates SS-CDC~\cite{sscdc},
which is another algorithm that connects adjacent segments
with parallelized BSW-based CDC.
The authors of SS-CDC focused on the exploitation of instruction-level parralelism,
through AVX instructions in particular,
which are available on modern processors.
In their experimental evaluation,
they concluded a speedup
that is much superior to existing systems like P-Dedupe,
and scales superlinearly with multiple CPU cores.
\leo{This is somewhat misleading because SIMD doesn't use multiple cores. Maybe they \emph{also} used multiple cores, but that's independent of instruction-level parallelism.}
\marcel{for me it reads like independent statements; suggestions?}
\leo{hmm. The more I think about this, the more it seems impossible. They can use SIMD instructions, which probably gives them a speedup per core. They can also use multiple cores, which gives them linear speedup in the number of cores. But combining this, they should still have a speedup in $\mathcal{O}(n)$ in the number of cores. They cannot get something like $\mathcal{O}(n^2)$, which I understand as superlinear...}

For the sake of completeness,
we also want to point out that there exist parallelization strategies 
which leverage features that are exclusive to GPUs
(\eg, Shredder~\cite{shredder}),
and that can further accelerate throughput.


==> sections/background/rechunking-stateful.tex <==
Lastly, we introduce a third class of algorithms. 
In 2020, Sardar and George proposed \ac{BFBC}~\cite{bfbc}.
This algorithm still iterates through a file byte-by-byte to determine the next cut-point,
but simplifies the matching condition using a simple table lookup: it checks if the current byte pair exists within a predefined set of byte-pair divisors.
The list of byte-pair divisors is derived from a statistical frequency analysis of byte pairs in the dataset,
performed once on a representative sample.
BFBC, therefore, tailors its matching condition to the expected data.
The simplification of the matching condition promises great improvements in throughput compared to the classical BSW algorithms.


%The approaches discussed so far present baseline \ac{CDC} algorithms that deterministically
%and content-dependendly split a file into variable- but similiar-sized chunks.
%Building on top of these methods, 
%researchers found strategies to enhance the deduplication performance of CDC,
%in exchange for added layers of complexity and overall efficiency.
%Specifically, this has been the result of rechunking and adaptive strategies
%which consider the current state of the file system.

%%% TTTD
%The first popular algorithm in the category of rechunking was TTTD~\cite{tttd},
%which specifically addressed the issue of chunk-size variance (or pathological chunk sizes),% with current algorithms at that time
%as well as its effect on deduplication.
%The core concept of TTTD is to rechunk chunks that turned out large with a softened condition,
%and then to coalesce adjacent chunks that turned out pathologically small.
%This aids deduplication through combating pathological chunk sizes.
%In contrast to enforcing minimum or maximum chunk sizes, however,
%chunking is still content dependent, and does not degrade to FSC.
%Many works have later adopted and enhanced upon this idea~\cite{fingerdiff,rabinPrimary,jasim2018new}.
%
%%% Bimodal
%Another application of rechunking is presented by \emph{Bimodal CDC}~\cite{bimodal}
%and its descendants~\cite{fbc,bfbc,anchorDrivenSubchunk,zhou2013hysteresis}.
%This set of algorithms follows a greedy strategy 
%of increasing granularity in selected regions 
%in an attempt to maximize data deduplication.
%To this end, it takes a look at already existing files
%and their chunk duplicates with the current file.
%Subsequently, the algorithms follow the basic intuition
%that when two files share a common chunk,
%there is a good chance for a subset of the directly adjacent non-duplicated chunks
%to contain more bytes that are duplicated in both files.

%% Stateful vs. stateless
%This is different from TTTD-based approaches 
%as the resulting set of chunks depends on the existing dataset
%(\ie, it is not deterministic for a given file input).
%Same as the frequency-based algorithms,
%this technique is in the category of \textit{stateful} (vs. \textit{stateless}) chunking algorithms.
%It is important to be aware of this distinction because stateful algorithms,
%although they generally result in better deduplication ratios,
%come at the cost of increased complexity and expensive existence queries.
%Depending on the environment (\eg, a distributed storage system),
%its performance can become impractical.

%%% FBC
%\ac{FBC}~\cite{fbc},
%and its improved version IFBC~\cite{zhang2013novel}, 
%represent stateful techniques for rechunking files to identify smaller globally duplicate blocks. 
%These algorithms leverage an efficient method based on Bloom filters to perform statistical chunk frequency estimations, enhancing the detection of duplicate data.
%The authors claim a deduplication ratio that is \qty{50}{\%} higher than what can be achieved with plain BSW.
%
%%% BFBC
%Recently, researchers proposed
%\ac{BFBC}~\cite{bfbc}
%which picks up on the ideas of statistical frequency estimations,
%yet is decisively different from the algorithm in \ac{FBC}.
%BFBC starts by conducting a statistical analysis on the dataset to determine the top most frequent byte pairs,
%which are then used as divisors in the file chunking process
%(while also employing minimum and maximum chunk size thresholds).
%In their experimental evaluation, \ac{BFBC} significantly outperformed the deduplication ratio achieved by TTTD.
%Furthermore, BFBC employs a sophisticated novel hashing strategy to identify duplicated chunks.
%This has further led to a high overall throughput,
%stating $10\times$ the performance of Rabin-based CDC.


==> sections/background/whole-file.tex <==
As previously stated, numerous studies~\cite{meyer2012study,el2012primary,wallace2012characteristics} 
have demonstrated the remarkable potential of block-based
data deduplication in primary and secondary storage systems.
However, files naturally occur duplicated on such systems, particularly in backup storages containing a series of disk snapshots. 
As a result, \emph{file}-level deduplication, which uses whole files as the unit of deduplication, can be an effective data reduction technique.
Furthermore, this approach benefits from decreased complexity
and circumvents the efficiency drawbacks that arise from the process of file chunking.
%\leo{does not understand what these efficiency drawbacks are. For file-level dedup we'd need to read and hash the whole file as well, no? So the assumption is that CDC is very slow, but that doesn't really hold...}
%\marcel{it's the expensive process of chunking that you save :D}

The effectiveness of whole-file vs. block-based deduplication depends on various factors, \eg,
how often the files change, or whether changes occur in small or large files.
Generally, however, file-level deduplication yields less effective space reduction due to its lack of granularity.
In the study conducted by Microsoft~\cite{meyer2012study}, 
file-level deduplication achieved only \qty{75}{\%} of the space savings that chunk-level deduplication was able to achieve on primary storage systems,
and \qty{87}{\%} on storages of backup disk images.
This result still demonstrates notable deduplication, 
and thus should be considered as an alternate option, 
contingent on the dataset and the resource economics of the system. 
Finally, the decision can be a question of
the overall size of the files, 
the frequency of file changes, 
and the frequency at which large files in particular change.

When opting for chunk-based deduplication, the size of the chunks has a critical impact on several performance metrics.
Its configuration therefore poses a crucial consideration for system designers.



==> sections/plots.tex <==


\begin{figure}
	\centering%
	\vspace{-0.2cm}%
	\input{fig/perf_quickcdc_rabin_variants_different_targets_code}\unskip%
	\vspace{-0.3cm}%
	\caption[Performance of QuickCDC around Rabin by Target Chunk Size]{
		Performance of QuickCDC around Rabin by Target Chunk Size, on the code dataset.
	}%
	\label{fig:perf_quickcdc_rabin_variants_different_targets_code}
\end{figure}

\begin{table*}
	\centering
	\input{tab/dedup_quickcdc_variants_all_datasets}
	\caption[Deduplication Ratio of QuickCDC Variants]{
		Deduplication Ratio of QuickCDC Variants on all datasets.
	}
	\label{tab:dedup_quickcdc_variants_all_datasets}
\end{table*}


\begin{table*}
	\centering
	\input{tab/csd_means_sd_buzhash}
	\caption[Chunk Size Distribution Summary for Buzhash Variants]{
		Chunk Size Distribution Summary for Buzhash Variants.
	}
	\label{tab:csd_means_sd_buzhash}
\end{table*}

\begin{table*}
	\centering
	\input{tab/csd_means_sd_bfbc}
	\caption[Chunk Size Distribution Summary for BFBC Variants]{
		Chunk Size Distribution Summary for BFBC Variants.
	}
	\label{tab:csd_means_sd_bfbc}
\end{table*}

\begin{table*}
	\centering
	\input{tab/csd_means_sd_gear}
	\caption[Chunk Size Distribution Summary for Gearhash Variants]{
		Chunk Size Distribution Summary for Gearhash Variants.
	}
	\label{tab:csd_means_sd_gear}
\end{table*}

\begin{table*}
	\centering
	\input{tab/csd_means_sd_rabin}
	\caption[Chunk Size Distribution Summary for Rabin Variants]{
		Chunk Size Distribution Summary for Rabin Variants.
	}
	\label{tab:csd_means_sd_rabin}
\end{table*}

\begin{table*}
	\centering
	\input{tab/csd_means_sd_adler32}
	\caption[Chunk Size Distribution Summary for Adler32 Variants]{
		Chunk Size Distribution Summary for Adler32 Variants.
	}
	\label{tab:csd_means_sd_adler32}
\end{table*}

\begin{table*}
	\centering
	\input{tab/csd_means_sd_quickcdc}
	\caption[Chunk Size Distribution Summary for QuickCDC Variants]{
		Chunk Size Distribution Summary for QuickCDC Variants.
	}
	\label{tab:csd_means_sd_quickcdc}
\end{table*}

\onecolumn
\begin{landscape}
	\input{tab/csd_means_sd_full}
\end{landscape}
\twocolumn


==> tab/csd_means_sd_adler32.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Tue Mar 28 19:23:09 2023
\begin{tabular}{llrrrrrrrrrr}
  \toprule
  && \multicolumn{2}{c}{512B} &\multicolumn{2}{c}{1KiB} &\multicolumn{2}{c}{2KiB} &\multicolumn{2}{c}{4KiB} &\multicolumn{2}{c}{8KiB}\\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
algorithm & dataset & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD\\ \midrule
adler32\_16 & random & 527 & 511.89 & 765 & 750.22 & 768 & 753.14 &  &  &  &  \\ 
  adler32\_32 & random & 544 & 512.73 & 998 & 966.87 & 1097 & 1066.05 & 1097 & 1066.05 &  &  \\ 
  adler32\_48 & random & 560 & 512.87 & 1068 & 1019.56 & 1355 & 1306.51 & 2310730 & 2332137.76 & 5546946 & 4838638.28 \\ 
  adler32\_64 & random & 576 & 513.02 & 1095 & 1031.37 & 1573 & 1509.09 & 1580 & 1516.77 & 1580 & 1516.77 \\ 
  adler32\_128 & random & 641 & 513.69 & 1162 & 1035.24 & 2084 & 1960.09 & 2292 & 2169.59 & 2292 & 2169.63 \\ 
  adler32\_256 & random & 1289 & 1035.46 & 1289 & 1035.46 & 2351 & 2097.43 & 3353 & 3100.23 & 3371 & 3118.41 \\ 
  adler32\_16 & code & 1316 & 2506.60 & 3510 & 6233.90 & 283761 & 4073131.00 &  &  &  &  \\ 
  adler32\_32 & code & 1142 & 7257.58 & 2382 & 9837.23 & 7297 & 22163.95 & 366965 & 6122915.93 &  &  \\ 
  adler32\_48 & code & 1089 & 6840.25 & 2017 & 8812.65 & 2838 & 11907.79 & 3603 & 15353.51 & 953654 & 10647413.17 \\ 
  adler32\_64 & code & 1036 & 1938.26 & 2259 & 9153.94 & 6093 & 17389.26 & 15348 & 67412.81 & 496125 & 7106220.32 \\ 
  adler32\_128 & code & 792 & 4404.94 & 1259 & 7692.77 & 4279 & 12988.03 & 16363 & 56403.27 & 30707 & 132563.77 \\ 
  adler32\_256 & code & 2052 & 8984.45 & 2052 & 8984.45 & 3865 & 11851.80 & 8533 & 19787.31 & 34269 & 101870.85 \\ 
  adler32\_16 & web & 638 & 1023.14 & 1150 & 2989.62 & 1824 & 28907.96 &  &  &  &  \\ 
  adler32\_32 & web & 634 & 800.82 & 1267 & 1707.08 & 1767 & 5840.38 & 2750 & 35103.42 &  &  \\ 
  adler32\_48 & web & 650 & 866.55 & 1280 & 1794.94 & 1800 & 3527.55 & 16844 & 98829.82 & 687769 & 1173678.43 \\ 
  adler32\_64 & web & 660 & 865.77 & 1406 & 2293.54 & 2351 & 4382.23 & 2958 & 12336.10 & 4578 & 42700.22 \\ 
  adler32\_128 & web & 694 & 649.63 & 1300 & 1493.55 & 2743 & 3770.52 & 3950 & 8451.74 & 4922 & 24858.81 \\ 
  adler32\_256 & web & 1472 & 1597.03 & 1472 & 1597.03 & 2931 & 3770.22 & 5341 & 8608.35 & 6891 & 18432.43 \\ 
  adler32\_16 & pdf & 562 & 2276.22 & 884 & 3081.78 & 986 & 5796.03 &  &  &  &  \\ 
  adler32\_32 & pdf & 547 & 833.56 & 1121 & 4005.55 & 1398 & 4590.65 & 1486 & 7113.25 &  &  \\ 
  adler32\_48 & pdf & 585 & 2196.44 & 1155 & 3310.05 & 1795 & 5951.80 & 32216 & 76360.42 & 144875 & 280499.17 \\ 
  adler32\_64 & pdf & 586 & 1185.12 & 1083 & 1975.32 & 1994 & 4866.86 & 2173 & 5335.82 & 2305 & 9306.00 \\ 
  adler32\_128 & pdf & 656 & 1744.94 & 1176 & 3523.65 & 2140 & 5149.38 & 3277 & 7673.44 & 3420 & 9862.94 \\ 
  adler32\_256 & pdf & 1317 & 3004.21 & 1317 & 3004.21 & 2372 & 4487.47 & 4092 & 6923.45 & 5404 & 10130.64 \\ 
  adler32\_16 & lnx & 532 & 1211.53 & 812 & 1692.68 & 823 & 4581.59 &  &  &  &  \\ 
  adler32\_32 & lnx & 548 & 1204.82 & 1032 & 1885.64 & 1222 & 2416.26 & 1224 & 5651.99 &  &  \\ 
  adler32\_48 & lnx & 565 & 1214.56 & 1084 & 1868.33 & 1532 & 2429.25 & 109348 & 303695.36 & 155456 & 578827.20 \\ 
  adler32\_64 & lnx & 580 & 1230.20 & 1106 & 1954.54 & 1764 & 2746.77 & 1851 & 4058.35 & 1854 & 7220.27 \\ 
  adler32\_128 & lnx & 644 & 1277.94 & 1169 & 1894.51 & 2177 & 3078.12 & 2801 & 4012.66 & 2852 & 5771.73 \\ 
  adler32\_256 & lnx & 1299 & 2069.96 & 1299 & 2069.96 & 2375 & 3219.51 & 3904 & 4884.27 & 4438 & 6430.25 \\ 
   \bottomrule
\end{tabular}


==> tab/csd_means_sd_bfbc.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Tue Mar 28 19:23:11 2023
\begin{tabular}{llrrrrrrrrrr}
  \toprule
  && \multicolumn{2}{c}{512B} &\multicolumn{2}{c}{1KiB} &\multicolumn{2}{c}{2KiB} &\multicolumn{2}{c}{4KiB} &\multicolumn{2}{c}{8KiB}\\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
algorithm & dataset & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD\\ \midrule
bfbc & random & 21750 & 21434.81 & 22268 & 21436.57 & 23292 & 21437.98 & 25347 & 21442.90 & 29468 & 21441.41 \\ 
  bfbc\_custom\_div & random & 513 & 511.20 & 1022 & 1020.14 & 2074 & 2071.34 & 4013 & 4009.63 & 8018 & 8012.18 \\ 
  bfbc & code & 594 & 4587.96 & 1245 & 7425.23 & 2473 & 12375.25 & 4786 & 15375.44 & 9312 & 20595.77 \\ 
  bfbc\_custom\_div & code & 2704 & 23436.29 & 2816 & 15402.04 & 17359 & 134380.09 & 15662 & 56680.64 & 35827 & 161864.27 \\ 
  bfbc & web & 3876 & 39419.28 & 5505 & 46127.61 & 7796 & 54502.74 & 11109 & 61737.77 & 16808 & 68652.25 \\ 
  bfbc\_custom\_div & web & 12298 & 79478.83 & 7102 & 23563.54 & 25253 & 38267.24 & 64644 & 154472.41 & 21537 & 33443.19 \\ 
  bfbc & pdf & 2492 & 8114.04 & 4276 & 10283.97 & 6653 & 12284.85 & 10102 & 14287.00 & 15772 & 16479.80 \\ 
  bfbc\_custom\_div & pdf & 964 & 9823.52 & 2401 & 14727.49 & 3519 & 18935.58 & 29538 & 87857.48 & 8236 & 40598.12 \\ 
  bfbc & lnx & 20560 & 36838.77 & 22787 & 38101.85 & 25226 & 39301.00 & 29022 & 40943.58 & 34780 & 43029.46 \\ 
  bfbc\_custom\_div & lnx & 767 & 1562.03 & 1937 & 3145.51 & 4796 & 7784.45 & 10983 & 20916.11 & 18667 & 42711.18 \\ 
   \bottomrule
\end{tabular}


==> tab/csd_means_sd_buzhash.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Tue Mar 28 19:23:08 2023
\begin{tabular}{llrrrrrrrrrr}
  \toprule
  && \multicolumn{2}{c}{512B} &\multicolumn{2}{c}{1KiB} &\multicolumn{2}{c}{2KiB} &\multicolumn{2}{c}{4KiB} &\multicolumn{2}{c}{8KiB}\\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
algorithm & dataset & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD\\ \midrule
buzhash\_16 & random & 527 & 511.77 & 1039 & 1023.35 & 2065 & 2048.00 & 4111 & 4097.94 & 8228 & 8229.53 \\ 
  buzhash\_32 & random & 544 & 512.08 & 1057 & 1024.75 & 2083 & 2050.29 & 4132 & 4099.10 & 8234 & 8193.97 \\ 
  buzhash\_48 & random & 559 & 511.79 & 1071 & 1022.82 & 2096 & 2047.83 & 4149 & 4113.26 & 8253 & 8216.64 \\ 
  buzhash\_64 & random & 575 & 511.52 & 1088 & 1024.84 & 2115 & 2053.86 & 4168 & 4112.79 & 8287 & 8233.85 \\ 
  buzhash\_128 & random & 639 & 512.11 & 1152 & 1025.04 & 2178 & 2051.43 & 4232 & 4109.06 & 8327 & 8200.24 \\ 
  buzhash\_256 & random & 1280 & 1026.30 & 1280 & 1026.30 & 2307 & 2054.80 & 4356 & 4096.62 & 8444 & 8181.79 \\ 
  buzhash\_16 & code & 944 & 2399.55 & 1773 & 3366.73 & 3184 & 5339.59 & 8558 & 18780.95 & 17121 & 30199.40 \\ 
  buzhash\_32 & code & 732 & 2230.21 & 1129 & 2637.21 & 3755 & 12023.59 & 6634 & 16070.02 & 10993 & 22757.03 \\ 
  buzhash\_48 & code & 1032 & 1898.33 & 1873 & 2736.35 & 3620 & 4437.01 & 7346 & 16206.43 & 13824 & 23420.70 \\ 
  buzhash\_64 & code & 426 & 2145.18 & 605 & 2500.98 & 821 & 2937.72 & 1040 & 3588.45 & 1253 & 4664.84 \\ 
  buzhash\_128 & code & 571 & 441.97 & 802 & 806.51 & 1081 & 2980.64 & 1361 & 3657.61 & 1659 & 4818.65 \\ 
  buzhash\_256 & code & 1424 & 7624.15 & 1424 & 7624.15 & 2263 & 9001.99 & 3347 & 10507.94 & 4639 & 12367.21 \\ 
  buzhash\_16 & web & 610 & 671.76 & 1267 & 1572.75 & 2644 & 3214.35 & 5577 & 6383.06 & 12201 & 13775.71 \\ 
  buzhash\_32 & web & 574 & 552.47 & 1095 & 1077.29 & 2554 & 2694.63 & 5222 & 5367.06 & 11065 & 11338.37 \\ 
  buzhash\_48 & web & 624 & 625.83 & 1206 & 1227.41 & 2304 & 2337.23 & 4986 & 4937.54 & 10500 & 10653.59 \\ 
  buzhash\_64 & web & 550 & 506.06 & 992 & 1014.72 & 1710 & 2020.88 & 2998 & 4299.12 & 4456 & 7628.31 \\ 
  buzhash\_128 & web & 630 & 511.45 & 1078 & 1007.34 & 1861 & 1997.13 & 3066 & 3859.24 & 4692 & 7114.30 \\ 
  buzhash\_256 & web & 1265 & 1023.89 & 1265 & 1023.89 & 2289 & 2073.77 & 4269 & 4314.23 & 7731 & 8367.71 \\ 
  buzhash\_16 & pdf & 544 & 791.30 & 1080 & 1573.81 & 2127 & 2891.32 & 4222 & 5366.96 & 8684 & 10441.87 \\ 
  buzhash\_32 & pdf & 557 & 697.11 & 1073 & 1274.30 & 2069 & 2400.83 & 4193 & 4718.37 & 8075 & 9183.94 \\ 
  buzhash\_48 & pdf & 573 & 665.78 & 1102 & 1264.10 & 2165 & 2414.52 & 4277 & 4658.69 & 8482 & 9088.43 \\ 
  buzhash\_64 & pdf & 575 & 588.60 & 1067 & 1105.31 & 1990 & 2117.32 & 3644 & 4075.24 & 6321 & 7780.34 \\ 
  buzhash\_128 & pdf & 642 & 592.85 & 1150 & 1109.83 & 2136 & 2141.01 & 3997 & 4161.86 & 7339 & 8134.39 \\ 
  buzhash\_256 & pdf & 1286 & 1112.13 & 1286 & 1112.13 & 2306 & 2145.23 & 4287 & 4198.41 & 8037 & 8232.25 \\ 
  buzhash\_16 & lnx & 530 & 1182.60 & 1047 & 1889.76 & 2083 & 3055.87 & 4164 & 5264.58 & 8349 & 9660.39 \\ 
  buzhash\_32 & lnx & 547 & 1194.95 & 1065 & 1893.85 & 2103 & 3056.03 & 4186 & 5269.78 & 8382 & 9543.12 \\ 
  buzhash\_48 & lnx & 562 & 1206.90 & 1079 & 1832.96 & 2115 & 3054.41 & 4200 & 5235.11 & 8394 & 9509.76 \\ 
  buzhash\_64 & lnx & 576 & 513.19 & 1088 & 1026.26 & 2111 & 2051.43 & 4154 & 4110.23 & 8200 & 8226.22 \\ 
  buzhash\_128 & lnx & 640 & 513.49 & 1153 & 1027.55 & 2179 & 2056.46 & 4227 & 4112.35 & 8283 & 8219.49 \\ 
  buzhash\_256 & lnx & 1281 & 1027.27 & 1281 & 1027.27 & 2307 & 2056.77 & 4359 & 4123.51 & 8429 & 8230.76 \\ 
   \bottomrule
\end{tabular}


==> tab/csd_means_sd_gear.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Tue Mar 28 19:23:10 2023
\begin{tabular}{llrrrrrrrrrr}
  \toprule
  && \multicolumn{2}{c}{512B} &\multicolumn{2}{c}{1KiB} &\multicolumn{2}{c}{2KiB} &\multicolumn{2}{c}{4KiB} &\multicolumn{2}{c}{8KiB}\\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
algorithm & dataset & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD\\ \midrule
gear & random & 513 & 510.76 & 1025 & 1023.64 & 2049 & 2050.17 & 4095 & 4097.69 & 8189 & 8177.79 \\ 
  gear\_nc\_1 & random & 559 & 339.47 & 1117 & 680.19 & 2231 & 1362.71 & 4466 & 2729.71 & 8937 & 5453.65 \\ 
  gear\_nc\_2 & random & 553 & 210.30 & 1105 & 420.48 & 2210 & 841.05 & 4421 & 1684.97 & 8852 & 3374.43 \\ 
  gear\_nc\_3 & random & 538 & 130.31 & 1076 & 261.46 & 2150 & 522.75 & 4299 & 1047.57 & 8602 & 2097.93 \\ 
  gear64 & random & 537 & 534.58 & 1071 & 1067.42 & 2130 & 2129.65 & 4254 & 4255.21 & 8510 & 8505.25 \\ 
  gear64\_simd & random & 537 & 534.58 & 1071 & 1067.42 & 2130 & 2129.65 & 4254 & 4255.21 & 8510 & 8505.25 \\ 
  gear & code & 1085 & 6817.28 & 1950 & 8595.42 & 3522 & 10988.54 & 7790 & 17130.67 & 14298 & 25462.67 \\ 
  gear\_nc\_1 & code & 897 & 6422.89 & 1691 & 8107.53 & 3234 & 10746.38 & 6055 & 13926.84 & 12601 & 20409.14 \\ 
  gear\_nc\_2 & code & 710 & 5812.92 & 1443 & 7825.51 & 2775 & 9998.29 & 5320 & 12939.39 & 10524 & 17179.22 \\ 
  gear\_nc\_3 & code & 601 & 197.45 & 1230 & 7176.19 & 2458 & 9389.23 & 4841 & 12242.08 & 9493 & 16086.59 \\ 
  gear64 & code & 935 & 6381.60 & 1696 & 8315.80 & 3234 & 10884.74 & 7107 & 16040.75 & 13739 & 23325.26 \\ 
  gear64\_simd & code & 935 & 6381.60 & 1696 & 8315.80 & 3234 & 10884.74 & 7107 & 16040.75 & 13739 & 23325.26 \\ 
  gear & web & 589 & 664.11 & 1200 & 1277.94 & 2442 & 2476.05 & 5121 & 5118.61 & 10816 & 10275.11 \\ 
  gear\_nc\_1 & web & 605 & 415.85 & 1227 & 843.20 & 2456 & 1582.92 & 4949 & 3050.92 & 10433 & 6107.77 \\ 
  gear\_nc\_2 & web & 572 & 233.96 & 1159 & 501.05 & 2338 & 983.13 & 4724 & 1844.29 & 9635 & 3455.38 \\ 
  gear\_nc\_3 & web & 548 & 148.18 & 1096 & 285.48 & 2226 & 580.79 & 4496 & 1138.13 & 8974 & 2024.70 \\ 
  gear64 & web & 573 & 580.20 & 1113 & 1119.29 & 2435 & 2593.64 & 5559 & 5617.20 & 11997 & 11714.90 \\ 
  gear64\_simd & web & 573 & 580.20 & 1113 & 1119.29 & 2435 & 2593.64 & 5559 & 5617.20 & 11997 & 11714.90 \\ 
  gear & pdf & 520 & 677.67 & 1034 & 1288.40 & 2003 & 2385.80 & 3898 & 4664.42 & 8547 & 9486.35 \\ 
  gear\_nc\_1 & pdf & 565 & 542.51 & 1112 & 947.56 & 2189 & 1777.58 & 4557 & 3247.03 & 9106 & 6338.25 \\ 
  gear\_nc\_2 & pdf & 556 & 438.83 & 1101 & 725.41 & 2243 & 1229.59 & 4483 & 2263.15 & 8924 & 4121.56 \\ 
  gear\_nc\_3 & pdf & 540 & 339.22 & 1087 & 590.18 & 2172 & 951.05 & 4336 & 1606.90 & 8647 & 2948.34 \\ 
  gear64 & pdf & 553 & 687.84 & 1102 & 1312.03 & 2193 & 2490.41 & 4365 & 4848.08 & 8806 & 9544.68 \\ 
  gear64\_simd & pdf & 553 & 687.84 & 1102 & 1312.03 & 2193 & 2490.41 & 4365 & 4848.08 & 8806 & 9544.68 \\ 
  gear & lnx & 516 & 1164.33 & 1033 & 1811.27 & 2069 & 3051.78 & 4154 & 5550.73 & 8343 & 9857.25 \\ 
  gear\_nc\_1 & lnx & 561 & 1134.10 & 1123 & 1682.85 & 2247 & 2582.47 & 4500 & 4286.03 & 9032 & 7696.89 \\ 
  gear\_nc\_2 & lnx & 556 & 1095.63 & 1110 & 1574.87 & 2220 & 2313.42 & 4446 & 3774.24 & 8894 & 5690.87 \\ 
  gear\_nc\_3 & lnx & 540 & 1072.85 & 1080 & 1516.33 & 2158 & 2167.90 & 4317 & 3307.04 & 8640 & 5278.19 \\ 
  gear64 & lnx & 540 & 1194.91 & 1079 & 1858.02 & 2152 & 3050.62 & 4318 & 5400.42 & 8661 & 9823.44 \\ 
  gear64\_simd & lnx & 540 & 1194.91 & 1079 & 1858.02 & 2152 & 3050.62 & 4318 & 5400.42 & 8661 & 9823.44 \\ 
   \bottomrule
\end{tabular}


==> tab/csd_means_sd_quickcdc.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Tue Mar 28 19:23:07 2023
\begin{tabular}{llrrrrrrrrrr}
  \toprule
  && \multicolumn{2}{c}{512B} &\multicolumn{2}{c}{1KiB} &\multicolumn{2}{c}{2KiB} &\multicolumn{2}{c}{4KiB} &\multicolumn{2}{c}{8KiB}\\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
algorithm & dataset & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD\\ \midrule
fsc & random & 512 & 0.00 & 1024 & 0.00 & 2048 & 0.00 & 4096 & 0.00 & 8192 & 0.00 \\ 
  ae & random & 446 & 122.80 & 806 & 184.67 & 1439 & 237.85 & 2639 & 255.47 & 5023 & 256.27 \\ 
  ram & random & 509 & 231.53 & 839 & 249.19 & 1446 & 254.94 & 2640 & 255.99 & 5024 & 256.29 \\ 
  mii & random & 609 & 366.83 & 800 & 644.36 & 879 & 841.64 & 4564 & 2933.94 & 5794 & 4891.23 \\ 
  pci & random & 563 & 519.34 & 1111 & 1065.27 & 2160 & 2115.03 & 4118 & 4078.55 & 8281 & 8235.19 \\ 
  rabin\_16 & random & 527 & 511.02 & 1039 & 1023.12 & 2064 & 2044.82 & 4108 & 4094.42 & 8189 & 8195.26 \\ 
  rabin\_32 & random & 543 & 511.25 & 1055 & 1023.85 & 2078 & 2046.80 & 4126 & 4101.78 & 8227 & 8200.86 \\ 
  rabin\_48 & random & 559 & 511.31 & 1071 & 1021.72 & 2094 & 2045.97 & 4138 & 4091.05 & 8238 & 8157.35 \\ 
  rabin\_64 & random & 576 & 511.95 & 1088 & 1023.76 & 2112 & 2048.03 & 4161 & 4087.81 & 8232 & 8150.60 \\ 
  rabin\_128 & random & 639 & 511.02 & 1151 & 1021.85 & 2173 & 2042.64 & 4218 & 4094.00 & 8325 & 8195.32 \\ 
  rabin\_256 & random & 1281 & 1023.50 & 1281 & 1023.50 & 2306 & 2049.60 & 4353 & 4097.77 & 8469 & 8173.44 \\ 
  adler32\_16 & random & 527 & 511.89 & 765 & 750.22 & 768 & 753.14 &  &  &  &  \\ 
  adler32\_32 & random & 544 & 512.73 & 998 & 966.87 & 1097 & 1066.05 & 1097 & 1066.05 &  &  \\ 
  adler32\_48 & random & 560 & 512.87 & 1068 & 1019.56 & 1355 & 1306.51 & 2310730 & 2332137.76 & 5546946 & 4838638.28 \\ 
  adler32\_64 & random & 576 & 513.02 & 1095 & 1031.37 & 1573 & 1509.09 & 1580 & 1516.77 & 1580 & 1516.77 \\ 
  adler32\_128 & random & 641 & 513.69 & 1162 & 1035.24 & 2084 & 1960.09 & 2292 & 2169.59 & 2292 & 2169.63 \\ 
  adler32\_256 & random & 1289 & 1035.46 & 1289 & 1035.46 & 2351 & 2097.43 & 3353 & 3100.23 & 3371 & 3118.41 \\ 
  buzhash\_16 & random & 527 & 511.77 & 1039 & 1023.35 & 2065 & 2048.00 & 4111 & 4097.94 & 8228 & 8229.53 \\ 
  buzhash\_32 & random & 544 & 512.08 & 1057 & 1024.75 & 2083 & 2050.29 & 4132 & 4099.10 & 8234 & 8193.97 \\ 
  buzhash\_48 & random & 559 & 511.79 & 1071 & 1022.82 & 2096 & 2047.83 & 4149 & 4113.26 & 8253 & 8216.64 \\ 
  buzhash\_64 & random & 575 & 511.52 & 1088 & 1024.84 & 2115 & 2053.86 & 4168 & 4112.79 & 8287 & 8233.85 \\ 
  buzhash\_128 & random & 639 & 512.11 & 1152 & 1025.04 & 2178 & 2051.43 & 4232 & 4109.06 & 8327 & 8200.24 \\ 
  buzhash\_256 & random & 1280 & 1026.30 & 1280 & 1026.30 & 2307 & 2054.80 & 4356 & 4096.62 & 8444 & 8181.79 \\ 
  gear & random & 513 & 510.76 & 1025 & 1023.64 & 2049 & 2050.17 & 4095 & 4097.69 & 8189 & 8177.79 \\ 
  gear\_nc\_1 & random & 559 & 339.47 & 1117 & 680.19 & 2231 & 1362.71 & 4466 & 2729.71 & 8937 & 5453.65 \\ 
  gear\_nc\_2 & random & 553 & 210.30 & 1105 & 420.48 & 2210 & 841.05 & 4421 & 1684.97 & 8852 & 3374.43 \\ 
  gear\_nc\_3 & random & 538 & 130.31 & 1076 & 261.46 & 2150 & 522.75 & 4299 & 1047.57 & 8602 & 2097.93 \\ 
  gear64 & random & 537 & 534.58 & 1071 & 1067.42 & 2130 & 2129.65 & 4254 & 4255.21 & 8510 & 8505.25 \\ 
  gear64\_simd & random & 537 & 534.58 & 1071 & 1067.42 & 2130 & 2129.65 & 4254 & 4255.21 & 8510 & 8505.25 \\ 
  quick\_2 & random & 559 & 339.47 & 1117 & 680.19 & 2231 & 1362.71 & 4466 & 2729.71 & 8937 & 5453.65 \\ 
  quick\_3 & random & 559 & 339.47 & 1117 & 680.19 & 2231 & 1362.71 & 4466 & 2729.71 & 8937 & 5453.65 \\ 
  quick\_hash\_2 & random & 559 & 339.47 & 1117 & 680.19 & 2231 & 1362.71 & 4466 & 2729.71 & 8937 & 5453.65 \\ 
  quick\_hash\_3 & random & 559 & 339.47 & 1117 & 680.19 & 2231 & 1362.71 & 4466 & 2729.71 & 8937 & 5453.65 \\ 
  bfbc & random & 21750 & 21434.81 & 22268 & 21436.57 & 23292 & 21437.98 & 25347 & 21442.90 & 29468 & 21441.41 \\ 
  bfbc\_custom\_div & random & 513 & 511.20 & 1022 & 1020.14 & 2074 & 2071.34 & 4013 & 4009.63 & 8018 & 8012.18 \\ 
  fsc & code & 512 & 0.00 & 1024 & 0.00 & 2048 & 0.00 & 4096 & 0.00 & 8192 & 0.00 \\ 
  ae & code & 462 & 150.13 & 927 & 289.88 & 1648 & 495.38 & 3048 & 802.18 & 5831 & 1451.93 \\ 
  ram & code & 55484 & 1467691.50 & 89741 & 1795938.97 & 114581 & 2033809.32 & 177169 & 2648271.71 & 291067 & 3461884.36 \\ 
  mii & code & 755 & 369.72 & 1159 & 798.20 & 1513 & 1433.62 & 4901 & 3326.10 & 6821 & 6485.15 \\ 
  pci & code & 22826 & 122037.38 & 45534 & 217500.45 & 77727 & 333307.71 & 130606 & 515843.83 & 189339 & 680225.59 \\ 
  rabin\_16 & code & 290 & 1918.68 & 379 & 2207.05 & 479 & 2633.14 & 591 & 3446.65 & 695 & 4783.34 \\ 
  rabin\_32 & code & 304 & 1382.52 & 403 & 1625.57 & 512 & 2012.13 & 622 & 2642.79 & 734 & 3640.43 \\ 
  rabin\_48 & code & 368 & 2015.56 & 507 & 2319.48 & 655 & 2700.37 & 820 & 3303.74 & 979 & 4279.17 \\ 
  rabin\_64 & code & 423 & 444.86 & 607 & 821.15 & 817 & 1437.53 & 1044 & 3594.69 & 1269 & 4678.56 \\ 
  rabin\_128 & code & 557 & 2173.02 & 798 & 2509.45 & 1071 & 2944.04 & 1367 & 3605.08 & 1652 & 4682.78 \\ 
  rabin\_256 & code & 1323 & 2705.10 & 1323 & 2705.10 & 2080 & 3432.96 & 3236 & 4688.67 & 4598 & 11330.70 \\ 
  adler32\_16 & code & 1316 & 2506.60 & 3510 & 6233.90 & 283761 & 4073131.00 &  &  &  &  \\ 
  adler32\_32 & code & 1142 & 7257.58 & 2382 & 9837.23 & 7297 & 22163.95 & 366965 & 6122915.93 &  &  \\ 
  adler32\_48 & code & 1089 & 6840.25 & 2017 & 8812.65 & 2838 & 11907.79 & 3603 & 15353.51 & 953654 & 10647413.17 \\ 
  adler32\_64 & code & 1036 & 1938.26 & 2259 & 9153.94 & 6093 & 17389.26 & 15348 & 67412.81 & 496125 & 7106220.32 \\ 
  adler32\_128 & code & 792 & 4404.94 & 1259 & 7692.77 & 4279 & 12988.03 & 16363 & 56403.27 & 30707 & 132563.77 \\ 
  adler32\_256 & code & 2052 & 8984.45 & 2052 & 8984.45 & 3865 & 11851.80 & 8533 & 19787.31 & 34269 & 101870.85 \\ 
  buzhash\_16 & code & 944 & 2399.55 & 1773 & 3366.73 & 3184 & 5339.59 & 8558 & 18780.95 & 17121 & 30199.40 \\ 
  buzhash\_32 & code & 732 & 2230.21 & 1129 & 2637.21 & 3755 & 12023.59 & 6634 & 16070.02 & 10993 & 22757.03 \\ 
  buzhash\_48 & code & 1032 & 1898.33 & 1873 & 2736.35 & 3620 & 4437.01 & 7346 & 16206.43 & 13824 & 23420.70 \\ 
  buzhash\_64 & code & 426 & 2145.18 & 605 & 2500.98 & 821 & 2937.72 & 1040 & 3588.45 & 1253 & 4664.84 \\ 
  buzhash\_128 & code & 571 & 441.97 & 802 & 806.51 & 1081 & 2980.64 & 1361 & 3657.61 & 1659 & 4818.65 \\ 
  buzhash\_256 & code & 1424 & 7624.15 & 1424 & 7624.15 & 2263 & 9001.99 & 3347 & 10507.94 & 4639 & 12367.21 \\ 
  gear & code & 1085 & 6817.28 & 1950 & 8595.42 & 3522 & 10988.54 & 7790 & 17130.67 & 14298 & 25462.67 \\ 
  gear\_nc\_1 & code & 897 & 6422.89 & 1691 & 8107.53 & 3234 & 10746.38 & 6055 & 13926.84 & 12601 & 20409.14 \\ 
  gear\_nc\_2 & code & 710 & 5812.92 & 1443 & 7825.51 & 2775 & 9998.29 & 5320 & 12939.39 & 10524 & 17179.22 \\ 
  gear\_nc\_3 & code & 601 & 197.45 & 1230 & 7176.19 & 2458 & 9389.23 & 4841 & 12242.08 & 9493 & 16086.59 \\ 
  gear64 & code & 935 & 6381.60 & 1696 & 8315.80 & 3234 & 10884.74 & 7107 & 16040.75 & 13739 & 23325.26 \\ 
  gear64\_simd & code & 935 & 6381.60 & 1696 & 8315.80 & 3234 & 10884.74 & 7107 & 16040.75 & 13739 & 23325.26 \\ 
  quick\_2 & code & 897 & 6422.89 & 1691 & 8107.53 & 3234 & 10746.38 & 6055 & 13926.84 & 12601 & 20409.14 \\ 
  quick\_3 & code & 897 & 6422.89 & 1691 & 8107.53 & 3234 & 10746.38 & 6055 & 13926.84 & 12601 & 20409.14 \\ 
  quick\_hash\_2 & code & 897 & 6422.89 & 1691 & 8107.53 & 3234 & 10746.38 & 6055 & 13926.84 & 12601 & 20409.14 \\ 
  quick\_hash\_3 & code & 897 & 6422.89 & 1691 & 8107.53 & 3234 & 10746.38 & 6055 & 13926.84 & 12601 & 20409.14 \\ 
  bfbc & code & 594 & 4587.96 & 1245 & 7425.23 & 2473 & 12375.25 & 4786 & 15375.44 & 9312 & 20595.77 \\ 
  bfbc\_custom\_div & code & 2704 & 23436.29 & 2816 & 15402.04 & 17359 & 134380.09 & 15662 & 56680.64 & 35827 & 161864.27 \\ 
  fsc & web & 512 & 0.00 & 1024 & 0.00 & 2048 & 0.00 & 4096 & 0.00 & 8192 & 0.00 \\ 
  ae & web & 453 & 135.09 & 817 & 202.90 & 1514 & 377.64 & 2772 & 522.11 & 5252 & 781.96 \\ 
  ram & web & 789 & 21970.17 & 1282 & 28030.23 & 2153 & 37040.37 & 3788 & 48438.00 & 6904 & 63368.46 \\ 
  mii & web & 638 & 371.21 & 874 & 694.46 & 1019 & 1043.24 & 5142 & 2997.73 & 7312 & 5684.80 \\ 
  pci & web & 770 & 5039.67 & 1425 & 8075.93 & 2433 & 13782.33 & 4093 & 20192.92 & 6302 & 27544.24 \\ 
  rabin\_16 & web & 525 & 587.60 & 972 & 1146.44 & 1717 & 2277.90 & 2912 & 5768.56 & 4241 & 10248.97 \\ 
  rabin\_32 & web & 539 & 552.99 & 983 & 1081.10 & 1716 & 2130.16 & 2784 & 4106.95 & 4031 & 7320.52 \\ 
  rabin\_48 & web & 553 & 558.27 & 1005 & 1098.49 & 1772 & 2125.23 & 3003 & 4641.80 & 4462 & 8313.52 \\ 
  rabin\_64 & web & 576 & 572.44 & 1037 & 1123.55 & 1836 & 2197.48 & 3097 & 4402.49 & 4701 & 7899.03 \\ 
  rabin\_128 & web & 627 & 523.53 & 1064 & 1022.14 & 1795 & 1993.71 & 2863 & 3811.23 & 4151 & 6797.67 \\ 
  rabin\_256 & web & 1314 & 1058.66 & 1314 & 1058.66 & 2386 & 2187.21 & 4609 & 4562.20 & 8533 & 8473.59 \\ 
  adler32\_16 & web & 638 & 1023.14 & 1150 & 2989.62 & 1824 & 28907.96 &  &  &  &  \\ 
  adler32\_32 & web & 634 & 800.82 & 1267 & 1707.08 & 1767 & 5840.38 & 2750 & 35103.42 &  &  \\ 
  adler32\_48 & web & 650 & 866.55 & 1280 & 1794.94 & 1800 & 3527.55 & 16844 & 98829.82 & 687769 & 1173678.43 \\ 
  adler32\_64 & web & 660 & 865.77 & 1406 & 2293.54 & 2351 & 4382.23 & 2958 & 12336.10 & 4578 & 42700.22 \\ 
  adler32\_128 & web & 694 & 649.63 & 1300 & 1493.55 & 2743 & 3770.52 & 3950 & 8451.74 & 4922 & 24858.81 \\ 
  adler32\_256 & web & 1472 & 1597.03 & 1472 & 1597.03 & 2931 & 3770.22 & 5341 & 8608.35 & 6891 & 18432.43 \\ 
  buzhash\_16 & web & 610 & 671.76 & 1267 & 1572.75 & 2644 & 3214.35 & 5577 & 6383.06 & 12201 & 13775.71 \\ 
  buzhash\_32 & web & 574 & 552.47 & 1095 & 1077.29 & 2554 & 2694.63 & 5222 & 5367.06 & 11065 & 11338.37 \\ 
  buzhash\_48 & web & 624 & 625.83 & 1206 & 1227.41 & 2304 & 2337.23 & 4986 & 4937.54 & 10500 & 10653.59 \\ 
  buzhash\_64 & web & 550 & 506.06 & 992 & 1014.72 & 1710 & 2020.88 & 2998 & 4299.12 & 4456 & 7628.31 \\ 
  buzhash\_128 & web & 630 & 511.45 & 1078 & 1007.34 & 1861 & 1997.13 & 3066 & 3859.24 & 4692 & 7114.30 \\ 
  buzhash\_256 & web & 1265 & 1023.89 & 1265 & 1023.89 & 2289 & 2073.77 & 4269 & 4314.23 & 7731 & 8367.71 \\ 
  gear & web & 589 & 664.11 & 1200 & 1277.94 & 2442 & 2476.05 & 5121 & 5118.61 & 10816 & 10275.11 \\ 
  gear\_nc\_1 & web & 605 & 415.85 & 1227 & 843.20 & 2456 & 1582.92 & 4949 & 3050.92 & 10433 & 6107.77 \\ 
  gear\_nc\_2 & web & 572 & 233.96 & 1159 & 501.05 & 2338 & 983.13 & 4724 & 1844.29 & 9635 & 3455.38 \\ 
  gear\_nc\_3 & web & 548 & 148.18 & 1096 & 285.48 & 2226 & 580.79 & 4496 & 1138.13 & 8974 & 2024.70 \\ 
  gear64 & web & 573 & 580.20 & 1113 & 1119.29 & 2435 & 2593.64 & 5559 & 5617.20 & 11997 & 11714.90 \\ 
  gear64\_simd & web & 573 & 580.20 & 1113 & 1119.29 & 2435 & 2593.64 & 5559 & 5617.20 & 11997 & 11714.90 \\ 
  quick\_2 & web & 605 & 415.85 & 1227 & 843.20 & 2456 & 1582.92 & 4949 & 3050.92 & 10433 & 6107.77 \\ 
  quick\_3 & web & 605 & 415.85 & 1227 & 843.20 & 2456 & 1582.92 & 4949 & 3050.92 & 10433 & 6107.77 \\ 
  quick\_hash\_2 & web & 605 & 415.85 & 1227 & 843.20 & 2456 & 1582.92 & 4949 & 3050.92 & 10433 & 6107.77 \\ 
  quick\_hash\_3 & web & 605 & 415.85 & 1227 & 843.20 & 2456 & 1582.92 & 4949 & 3050.92 & 10433 & 6107.77 \\ 
  bfbc & web & 3876 & 39419.28 & 5505 & 46127.61 & 7796 & 54502.74 & 11109 & 61737.77 & 16808 & 68652.25 \\ 
  bfbc\_custom\_div & web & 12298 & 79478.83 & 7102 & 23563.54 & 25253 & 38267.24 & 64644 & 154472.41 & 21537 & 33443.19 \\ 
  fsc & pdf & 512 & 0.00 & 1024 & 0.00 & 2048 & 0.00 & 4096 & 0.00 & 8192 & 0.00 \\ 
  ae & pdf & 442 & 130.82 & 813 & 209.67 & 1479 & 311.16 & 2722 & 433.51 & 5163 & 686.54 \\ 
  ram & pdf & 582 & 4163.40 & 956 & 5352.12 & 1633 & 6980.78 & 2932 & 9333.45 & 5493 & 12634.00 \\ 
  mii & pdf & 583 & 377.03 & 753 & 664.21 & 829 & 905.27 & 3761 & 3164.32 & 4551 & 5022.47 \\ 
  pci & pdf & 271 & 2701.00 & 360 & 3238.91 & 459 & 3754.07 & 575 & 4327.10 & 721 & 5092.20 \\ 
  rabin\_16 & pdf & 537 & 743.05 & 1034 & 1322.39 & 1985 & 2461.52 & 3798 & 4927.50 & 6740 & 9562.00 \\ 
  rabin\_32 & pdf & 552 & 674.80 & 1068 & 1249.12 & 2104 & 2377.35 & 4062 & 4652.78 & 7650 & 9039.04 \\ 
  rabin\_48 & pdf & 569 & 668.60 & 1089 & 1227.07 & 2113 & 2366.88 & 4091 & 4580.18 & 7777 & 8818.69 \\ 
  rabin\_64 & pdf & 585 & 670.71 & 1102 & 1210.97 & 2124 & 2279.00 & 4102 & 4383.95 & 7846 & 8540.25 \\ 
  rabin\_128 & pdf & 645 & 630.20 & 1159 & 1189.95 & 2197 & 2259.14 & 4224 & 4354.70 & 8157 & 8522.05 \\ 
  rabin\_256 & pdf & 1290 & 1188.92 & 1290 & 1188.92 & 2318 & 2218.65 & 4372 & 4320.62 & 8364 & 8425.57 \\ 
  adler32\_16 & pdf & 562 & 2276.22 & 884 & 3081.78 & 986 & 5796.03 &  &  &  &  \\ 
  adler32\_32 & pdf & 547 & 833.56 & 1121 & 4005.55 & 1398 & 4590.65 & 1486 & 7113.25 &  &  \\ 
  adler32\_48 & pdf & 585 & 2196.44 & 1155 & 3310.05 & 1795 & 5951.80 & 32216 & 76360.42 & 144875 & 280499.17 \\ 
  adler32\_64 & pdf & 586 & 1185.12 & 1083 & 1975.32 & 1994 & 4866.86 & 2173 & 5335.82 & 2305 & 9306.00 \\ 
  adler32\_128 & pdf & 656 & 1744.94 & 1176 & 3523.65 & 2140 & 5149.38 & 3277 & 7673.44 & 3420 & 9862.94 \\ 
  adler32\_256 & pdf & 1317 & 3004.21 & 1317 & 3004.21 & 2372 & 4487.47 & 4092 & 6923.45 & 5404 & 10130.64 \\ 
  buzhash\_16 & pdf & 544 & 791.30 & 1080 & 1573.81 & 2127 & 2891.32 & 4222 & 5366.96 & 8684 & 10441.87 \\ 
  buzhash\_32 & pdf & 557 & 697.11 & 1073 & 1274.30 & 2069 & 2400.83 & 4193 & 4718.37 & 8075 & 9183.94 \\ 
  buzhash\_48 & pdf & 573 & 665.78 & 1102 & 1264.10 & 2165 & 2414.52 & 4277 & 4658.69 & 8482 & 9088.43 \\ 
  buzhash\_64 & pdf & 575 & 588.60 & 1067 & 1105.31 & 1990 & 2117.32 & 3644 & 4075.24 & 6321 & 7780.34 \\ 
  buzhash\_128 & pdf & 642 & 592.85 & 1150 & 1109.83 & 2136 & 2141.01 & 3997 & 4161.86 & 7339 & 8134.39 \\ 
  buzhash\_256 & pdf & 1286 & 1112.13 & 1286 & 1112.13 & 2306 & 2145.23 & 4287 & 4198.41 & 8037 & 8232.25 \\ 
  gear & pdf & 520 & 677.67 & 1034 & 1288.40 & 2003 & 2385.80 & 3898 & 4664.42 & 8547 & 9486.35 \\ 
  gear\_nc\_1 & pdf & 565 & 542.51 & 1112 & 947.56 & 2189 & 1777.58 & 4557 & 3247.03 & 9106 & 6338.25 \\ 
  gear\_nc\_2 & pdf & 556 & 438.83 & 1101 & 725.41 & 2243 & 1229.59 & 4483 & 2263.15 & 8924 & 4121.56 \\ 
  gear\_nc\_3 & pdf & 540 & 339.22 & 1087 & 590.18 & 2172 & 951.05 & 4336 & 1606.90 & 8647 & 2948.34 \\ 
  gear64 & pdf & 553 & 687.84 & 1102 & 1312.03 & 2193 & 2490.41 & 4365 & 4848.08 & 8806 & 9544.68 \\ 
  gear64\_simd & pdf & 553 & 687.84 & 1102 & 1312.03 & 2193 & 2490.41 & 4365 & 4848.08 & 8806 & 9544.68 \\ 
  quick\_2 & pdf & 565 & 542.51 & 1112 & 947.56 & 2189 & 1777.58 & 4557 & 3247.03 & 9106 & 6338.25 \\ 
  quick\_3 & pdf & 565 & 542.51 & 1112 & 947.56 & 2189 & 1777.58 & 4557 & 3247.03 & 9106 & 6338.25 \\ 
  quick\_hash\_2 & pdf & 565 & 542.51 & 1112 & 947.56 & 2189 & 1777.58 & 4557 & 3247.03 & 9106 & 6338.25 \\ 
  quick\_hash\_3 & pdf & 565 & 542.51 & 1112 & 947.56 & 2189 & 1777.58 & 4557 & 3247.03 & 9106 & 6338.25 \\ 
  bfbc & pdf & 2492 & 8114.04 & 4276 & 10283.97 & 6653 & 12284.85 & 10102 & 14287.00 & 15772 & 16479.80 \\ 
  bfbc\_custom\_div & pdf & 964 & 9823.52 & 2401 & 14727.49 & 3519 & 18935.58 & 29538 & 87857.48 & 8236 & 40598.12 \\ 
  fsc & lnx & 512 & 0.00 & 1024 & 0.00 & 2048 & 0.00 & 4096 & 0.00 & 8192 & 0.00 \\ 
  ae & lnx & 440 & 123.51 & 798 & 189.23 & 1438 & 256.51 & 2648 & 331.15 & 5041 & 395.55 \\ 
  ram & lnx & 506 & 1229.81 & 840 & 1584.34 & 1457 & 2065.35 & 2662 & 2760.65 & 5062 & 3852.91 \\ 
  mii & lnx & 618 & 368.51 & 821 & 658.90 & 911 & 886.07 & 4590 & 2965.54 & 5872 & 5018.31 \\ 
  pci & lnx & 254 & 2537.37 & 348 & 3005.91 & 453 & 3500.40 & 573 & 4065.94 & 721 & 4790.43 \\ 
  rabin\_16 & lnx & 525 & 513.46 & 1030 & 1029.51 & 2024 & 2067.14 & 3953 & 4133.81 & 7582 & 8259.14 \\ 
  rabin\_32 & lnx & 544 & 513.17 & 1055 & 1027.46 & 2077 & 2055.28 & 4115 & 4118.89 & 8144 & 8226.98 \\ 
  rabin\_48 & lnx & 560 & 512.92 & 1072 & 1027.22 & 2094 & 2055.30 & 4138 & 4117.35 & 8183 & 8239.95 \\ 
  rabin\_64 & lnx & 576 & 512.45 & 1088 & 1024.79 & 2111 & 2051.13 & 4151 & 4108.97 & 8195 & 8238.22 \\ 
  rabin\_128 & lnx & 640 & 512.74 & 1152 & 1026.23 & 2178 & 2057.17 & 4226 & 4117.85 & 8297 & 8236.26 \\ 
  rabin\_256 & lnx & 1281 & 1025.73 & 1281 & 1025.73 & 2306 & 2054.33 & 4352 & 4111.62 & 8408 & 8226.68 \\ 
  adler32\_16 & lnx & 532 & 1211.53 & 812 & 1692.68 & 823 & 4581.59 &  &  &  &  \\ 
  adler32\_32 & lnx & 548 & 1204.82 & 1032 & 1885.64 & 1222 & 2416.26 & 1224 & 5651.99 &  &  \\ 
  adler32\_48 & lnx & 565 & 1214.56 & 1084 & 1868.33 & 1532 & 2429.25 & 109348 & 303695.36 & 155456 & 578827.20 \\ 
  adler32\_64 & lnx & 580 & 1230.20 & 1106 & 1954.54 & 1764 & 2746.77 & 1851 & 4058.35 & 1854 & 7220.27 \\ 
  adler32\_128 & lnx & 644 & 1277.94 & 1169 & 1894.51 & 2177 & 3078.12 & 2801 & 4012.66 & 2852 & 5771.73 \\ 
  adler32\_256 & lnx & 1299 & 2069.96 & 1299 & 2069.96 & 2375 & 3219.51 & 3904 & 4884.27 & 4438 & 6430.25 \\ 
  buzhash\_16 & lnx & 530 & 1182.60 & 1047 & 1889.76 & 2083 & 3055.87 & 4164 & 5264.58 & 8349 & 9660.39 \\ 
  buzhash\_32 & lnx & 547 & 1194.95 & 1065 & 1893.85 & 2103 & 3056.03 & 4186 & 5269.78 & 8382 & 9543.12 \\ 
  buzhash\_48 & lnx & 562 & 1206.90 & 1079 & 1832.96 & 2115 & 3054.41 & 4200 & 5235.11 & 8394 & 9509.76 \\ 
  buzhash\_64 & lnx & 576 & 513.19 & 1088 & 1026.26 & 2111 & 2051.43 & 4154 & 4110.23 & 8200 & 8226.22 \\ 
  buzhash\_128 & lnx & 640 & 513.49 & 1153 & 1027.55 & 2179 & 2056.46 & 4227 & 4112.35 & 8283 & 8219.49 \\ 
  buzhash\_256 & lnx & 1281 & 1027.27 & 1281 & 1027.27 & 2307 & 2056.77 & 4359 & 4123.51 & 8429 & 8230.76 \\ 
  gear & lnx & 516 & 1164.33 & 1033 & 1811.27 & 2069 & 3051.78 & 4154 & 5550.73 & 8343 & 9857.25 \\ 
  gear\_nc\_1 & lnx & 561 & 1134.10 & 1123 & 1682.85 & 2247 & 2582.47 & 4500 & 4286.03 & 9032 & 7696.89 \\ 
  gear\_nc\_2 & lnx & 556 & 1095.63 & 1110 & 1574.87 & 2220 & 2313.42 & 4446 & 3774.24 & 8894 & 5690.87 \\ 
  gear\_nc\_3 & lnx & 540 & 1072.85 & 1080 & 1516.33 & 2158 & 2167.90 & 4317 & 3307.04 & 8640 & 5278.19 \\ 
  gear64 & lnx & 540 & 1194.91 & 1079 & 1858.02 & 2152 & 3050.62 & 4318 & 5400.42 & 8661 & 9823.44 \\ 
  gear64\_simd & lnx & 540 & 1194.91 & 1079 & 1858.02 & 2152 & 3050.62 & 4318 & 5400.42 & 8661 & 9823.44 \\ 
  quick\_2 & lnx & 561 & 1134.10 & 1123 & 1682.85 & 2247 & 2582.47 & 4500 & 4286.03 & 9032 & 7696.89 \\ 
  quick\_3 & lnx & 561 & 1134.10 & 1123 & 1682.85 & 2247 & 2582.47 & 4500 & 4286.03 & 9032 & 7696.89 \\ 
  quick\_hash\_2 & lnx & 561 & 1134.10 & 1123 & 1682.85 & 2247 & 2582.47 & 4500 & 4286.03 & 9032 & 7696.89 \\ 
  quick\_hash\_3 & lnx & 561 & 1134.10 & 1123 & 1682.85 & 2247 & 2582.47 & 4500 & 4286.03 & 9032 & 7696.89 \\ 
  bfbc & lnx & 20560 & 36838.77 & 22787 & 38101.85 & 25226 & 39301.00 & 29022 & 40943.58 & 34780 & 43029.46 \\ 
  bfbc\_custom\_div & lnx & 767 & 1562.03 & 1937 & 3145.51 & 4796 & 7784.45 & 10983 & 20916.11 & 18667 & 42711.18 \\ 
   \bottomrule
\end{tabular}


==> tab/csd_means_sd_rabin.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Tue Mar 28 19:23:07 2023
\begin{tabular}{llrrrrrrrrrr}
  \toprule
  && \multicolumn{2}{c}{512B} &\multicolumn{2}{c}{1KiB} &\multicolumn{2}{c}{2KiB} &\multicolumn{2}{c}{4KiB} &\multicolumn{2}{c}{8KiB}\\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}
algorithm & dataset & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD & $\mu$ & SD\\ \midrule
rabin\_16 & random & 527 & 511.02 & 1039 & 1023.12 & 2064 & 2044.82 & 4108 & 4094.42 & 8189 & 8195.26 \\ 
  rabin\_32 & random & 543 & 511.25 & 1055 & 1023.85 & 2078 & 2046.80 & 4126 & 4101.78 & 8227 & 8200.86 \\ 
  rabin\_48 & random & 559 & 511.31 & 1071 & 1021.72 & 2094 & 2045.97 & 4138 & 4091.05 & 8238 & 8157.35 \\ 
  rabin\_64 & random & 576 & 511.95 & 1088 & 1023.76 & 2112 & 2048.03 & 4161 & 4087.81 & 8232 & 8150.60 \\ 
  rabin\_128 & random & 639 & 511.02 & 1151 & 1021.85 & 2173 & 2042.64 & 4218 & 4094.00 & 8325 & 8195.32 \\ 
  rabin\_256 & random & 1281 & 1023.50 & 1281 & 1023.50 & 2306 & 2049.60 & 4353 & 4097.77 & 8469 & 8173.44 \\ 
  rabin\_16 & code & 290 & 1918.68 & 379 & 2207.05 & 479 & 2633.14 & 591 & 3446.65 & 695 & 4783.34 \\ 
  rabin\_32 & code & 304 & 1382.52 & 403 & 1625.57 & 512 & 2012.13 & 622 & 2642.79 & 734 & 3640.43 \\ 
  rabin\_48 & code & 368 & 2015.56 & 507 & 2319.48 & 655 & 2700.37 & 820 & 3303.74 & 979 & 4279.17 \\ 
  rabin\_64 & code & 423 & 444.86 & 607 & 821.15 & 817 & 1437.53 & 1044 & 3594.69 & 1269 & 4678.56 \\ 
  rabin\_128 & code & 557 & 2173.02 & 798 & 2509.45 & 1071 & 2944.04 & 1367 & 3605.08 & 1652 & 4682.78 \\ 
  rabin\_256 & code & 1323 & 2705.10 & 1323 & 2705.10 & 2080 & 3432.96 & 3236 & 4688.67 & 4598 & 11330.70 \\ 
  rabin\_16 & web & 525 & 587.60 & 972 & 1146.44 & 1717 & 2277.90 & 2912 & 5768.56 & 4241 & 10248.97 \\ 
  rabin\_32 & web & 539 & 552.99 & 983 & 1081.10 & 1716 & 2130.16 & 2784 & 4106.95 & 4031 & 7320.52 \\ 
  rabin\_48 & web & 553 & 558.27 & 1005 & 1098.49 & 1772 & 2125.23 & 3003 & 4641.80 & 4462 & 8313.52 \\ 
  rabin\_64 & web & 576 & 572.44 & 1037 & 1123.55 & 1836 & 2197.48 & 3097 & 4402.49 & 4701 & 7899.03 \\ 
  rabin\_128 & web & 627 & 523.53 & 1064 & 1022.14 & 1795 & 1993.71 & 2863 & 3811.23 & 4151 & 6797.67 \\ 
  rabin\_256 & web & 1314 & 1058.66 & 1314 & 1058.66 & 2386 & 2187.21 & 4609 & 4562.20 & 8533 & 8473.59 \\ 
  rabin\_16 & pdf & 537 & 743.05 & 1034 & 1322.39 & 1985 & 2461.52 & 3798 & 4927.50 & 6740 & 9562.00 \\ 
  rabin\_32 & pdf & 552 & 674.80 & 1068 & 1249.12 & 2104 & 2377.35 & 4062 & 4652.78 & 7650 & 9039.04 \\ 
  rabin\_48 & pdf & 569 & 668.60 & 1089 & 1227.07 & 2113 & 2366.88 & 4091 & 4580.18 & 7777 & 8818.69 \\ 
  rabin\_64 & pdf & 585 & 670.71 & 1102 & 1210.97 & 2124 & 2279.00 & 4102 & 4383.95 & 7846 & 8540.25 \\ 
  rabin\_128 & pdf & 645 & 630.20 & 1159 & 1189.95 & 2197 & 2259.14 & 4224 & 4354.70 & 8157 & 8522.05 \\ 
  rabin\_256 & pdf & 1290 & 1188.92 & 1290 & 1188.92 & 2318 & 2218.65 & 4372 & 4320.62 & 8364 & 8425.57 \\ 
  rabin\_16 & lnx & 525 & 513.46 & 1030 & 1029.51 & 2024 & 2067.14 & 3953 & 4133.81 & 7582 & 8259.14 \\ 
  rabin\_32 & lnx & 544 & 513.17 & 1055 & 1027.46 & 2077 & 2055.28 & 4115 & 4118.89 & 8144 & 8226.98 \\ 
  rabin\_48 & lnx & 560 & 512.92 & 1072 & 1027.22 & 2094 & 2055.30 & 4138 & 4117.35 & 8183 & 8239.95 \\ 
  rabin\_64 & lnx & 576 & 512.45 & 1088 & 1024.79 & 2111 & 2051.13 & 4151 & 4108.97 & 8195 & 8238.22 \\ 
  rabin\_128 & lnx & 640 & 512.74 & 1152 & 1026.23 & 2178 & 2057.17 & 4226 & 4117.85 & 8297 & 8236.26 \\ 
  rabin\_256 & lnx & 1281 & 1025.73 & 1281 & 1025.73 & 2306 & 2054.33 & 4352 & 4111.62 & 8408 & 8226.68 \\ 
   \bottomrule
\end{tabular}


==> tab/dedup_quickcdc_variants_all_datasets.tex <==
% latex table generated in R 4.2.3 by xtable 1.8-4 package
% Tue Jun 27 14:30:21 2023
\begin{tabular}{llrrrrr}
  \toprule
  && \multicolumn{5}{c}{Deduplication Ratio}\\
\cmidrule(lr){3-7}
algorithm & dataset & CS=512B & 1KiB & 2KiB & 4KiB & 8KiB\\ \midrule
rabin\_64 & code & 0.845872 & 0.825700 & 0.802335 & 0.774840 & 0.745259 \\ 
  quick\_2\_rabin\_64\_noskip & code & 0.822130 & 0.796013 & 0.765321 & 0.730793 & 0.695103 \\ 
  quick\_3\_rabin\_64\_noskip & code & 0.822600 & 0.796710 & 0.766173 & 0.731829 & 0.695983 \\ 
  rabin\_64 & lnx & 0.202422 & 0.200528 & 0.197158 & 0.191241 & 0.181959 \\ 
  quick\_2\_rabin\_64\_noskip & lnx & 0.201949 & 0.200033 & 0.196630 & 0.190548 & 0.181209 \\ 
  quick\_3\_rabin\_64\_noskip & lnx & 0.202249 & 0.200181 & 0.196712 & 0.190620 & 0.181267 \\ 
  rabin\_64 & pdf & 0.051860 & 0.046019 & 0.039081 & 0.032254 & 0.025902 \\ 
  quick\_2\_rabin\_64\_noskip & pdf & 0.051565 & 0.045453 & 0.038388 & 0.031501 & 0.025111 \\ 
  quick\_3\_rabin\_64\_noskip & pdf & 0.051691 & 0.045500 & 0.038452 & 0.031573 & 0.025195 \\ 
  rabin\_64 & web & 0.710056 & 0.704130 & 0.697314 & 0.687953 & 0.679110 \\ 
  quick\_2\_rabin\_64\_noskip & web & 0.708856 & 0.702908 & 0.695562 & 0.685755 & 0.675581 \\ 
  quick\_3\_rabin\_64\_noskip & web & 0.708892 & 0.702896 & 0.695988 & 0.686047 & 0.675878 \\ 
   \bottomrule
\end{tabular}


==> tab/perf_bfbc_vs_custom_bfbc_2kib.tex <==
% latex table generated in R 4.3.3 by xtable 1.8-4 package
% Mon Jul 29 13:02:14 2024
\begin{tabular}{llrrrrrr}
  \toprule
  && \multicolumn{2}{c}{\makecell{Throughput\\(MiB/s)}} & & &  & \\
\cmidrule(lr){3-4}
Alg. & Dataset & \rotatebox{90}{Median} & \rotatebox{90}{IQR} & \rotatebox{90}{Inst./B} & \rotatebox{90}{IPC} & \rotatebox{90}{Br./B} & \rotatebox{90}{BM-\%} \\ \midrule
BFBC & CODE & \num{876.0} & $7.6$ & \num{10.93} & \num{3.05} & \num{1.79} & \num{0.11} \\ 
  BFBC* & CODE & \num{585.2} & $6.7$ & \num{17.37} & \num{3.24} & \num{2.56} & \num{0.06} \\ 
  BFBC & RAND & \num{619.9} & $5.9$ & \num{16.78} & \num{3.24} & \num{2.49} & \num{0.05} \\ 
  BFBC* & RAND & \num{596.2} & $18.9$ & \num{17.38} & \num{3.24} & \num{2.56} & \num{0.06} \\ 
   \bottomrule
\end{tabular}


==> tab/perf_quickcdc_gear_variants.tex <==
% latex table generated in R 4.3.3 by xtable 1.8-4 package
% Fri May 17 13:45:53 2024
\begin{tabular}{llrrrrrrrrr}
  \toprule
  &&& \multicolumn{2}{c}{Throughput (MiB/s)} &
\multicolumn{2}{c}{Inst./B} &
\multicolumn{2}{c}{IPC} &
\multicolumn{2}{c}{L1D Miss (\%)}\\
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}
Algorithm & Dataset & Target (B) & Median & IQR & Mean & SE & Mean & SE & Mean & SE\\ \midrule
Gear NC-1 & CODE & $512$ & $499.4$ & $3.2$ & $16.48$ & $< 0.01$ & $2.57$ & $< 0.01$ & $0.54$ & $< 0.01$ \\ 
  Quick A-2 & CODE & $512$ & $789.6$ & $4.9$ & $9.3$ & $< 0.01$ & $2.15$ & $< 0.01$ & $2.13$ & $0.01$ \\ 
  Quick A-3 & CODE & $512$ & $743.7$ & $5.7$ & $9.32$ & $< 0.01$ & $2.03$ & $< 0.01$ & $2.33$ & $0.01$ \\ 
  Quick HM-2 & CODE & $512$ & $674.1$ & $5.8$ & $10.92$ & $< 0.01$ & $2.16$ & $< 0.01$ & $2.23$ & $0.01$ \\ 
  Quick HM-3 & CODE & $512$ & $701.3$ & $13.2$ & $11.01$ & $< 0.01$ & $2.24$ & $0.01$ & $2.26$ & $0.01$ \\ 
  Gear NC-1 & RAND & $512$ & $487.4$ & $5.4$ & $16.49$ & $< 0.01$ & $2.57$ & $< 0.01$ & $0.55$ & $0.01$ \\ 
  Quick A-2 & RAND & $512$ & $708.2$ & $17.4$ & $9.51$ & $< 0.01$ & $2.12$ & $< 0.01$ & $1.66$ & $0.01$ \\ 
  Quick A-3 & RAND & $512$ & $540.4$ & $6.4$ & $9.58$ & $< 0.01$ & $1.59$ & $0.01$ & $2.67$ & $0.01$ \\ 
  Quick HM-2 & RAND & $512$ & $590.4$ & $10.8$ & $11.17$ & $< 0.01$ & $2.06$ & $< 0.01$ & $1.98$ & $0.01$ \\ 
  Quick HM-3 & RAND & $512$ & $386.1$ & $4.3$ & $11.77$ & $< 0.01$ & $1.39$ & $< 0.01$ & $3.45$ & $0.01$ \\ 
  Gear NC-1 & CODE & $8{,}192$ & $516.7$ & $2.8$ & $16.36$ & $< 0.01$ & $2.58$ & $< 0.01$ & $0.55$ & $< 0.01$ \\ 
  Quick A-2 & CODE & $8{,}192$ & $812$ & $8.2$ & $9.01$ & $< 0.01$ & $2.15$ & $0.01$ & $2.18$ & $0.02$ \\ 
  Quick A-3 & CODE & $8{,}192$ & $812.8$ & $5.1$ & $8.88$ & $< 0.01$ & $2.12$ & $< 0.01$ & $2.24$ & $0.01$ \\ 
  Quick HM-2 & CODE & $8{,}192$ & $807.4$ & $6.5$ & $9.12$ & $< 0.01$ & $2.16$ & $< 0.01$ & $2.19$ & $0.02$ \\ 
  Quick HM-3 & CODE & $8{,}192$ & $920.6$ & $7.8$ & $8.98$ & $< 0.01$ & $2.45$ & $< 0.01$ & $2.22$ & $0.01$ \\ 
  Gear NC-1 & RAND & $8{,}192$ & $503.2$ & $16.8$ & $16.36$ & $< 0.01$ & $2.58$ & $< 0.01$ & $0.55$ & $< 0.01$ \\ 
  Quick A-2 & RAND & $8{,}192$ & $815.7$ & $28.7$ & $8.86$ & $< 0.01$ & $2.2$ & $< 0.01$ & $2.09$ & $0.01$ \\ 
  Quick A-3 & RAND & $8{,}192$ & $777.5$ & $16.9$ & $8.88$ & $< 0.01$ & $2.13$ & $< 0.01$ & $2.09$ & $0.01$ \\ 
  Quick HM-2 & RAND & $8{,}192$ & $778.9$ & $7.4$ & $8.97$ & $< 0.01$ & $2.18$ & $< 0.01$ & $2.14$ & $0.02$ \\ 
  Quick HM-3 & RAND & $8{,}192$ & $878.1$ & $9.7$ & $9.04$ & $< 0.01$ & $2.42$ & $0.01$ & $2.09$ & $0.02$ \\ 
   \bottomrule
\end{tabular}


==> tab/perf_quickcdc_rabin_variants.tex <==
% latex table generated in R 4.3.3 by xtable 1.8-4 package
% Sat May 18 08:35:33 2024
\begin{tabular}{llrrrrrrrrr}
  \toprule
  &&& \multicolumn{2}{c}{Throughput (MiB/s)} &
\multicolumn{2}{c}{Inst./B} &
\multicolumn{2}{c}{IPC} &
\multicolumn{2}{c}{L1 DCache Miss (\%)}\\
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}
Algorithm & Dataset & Target CS & Median & IQR & Mean & SE & Mean & SE & Mean & SE\\ \midrule
Rabin & CODE & $512$ & $204.6$ & $4.0$ & $34.11$ & $< 0.01$ & $2.2$ & $< 0.01$ & $0.15$ & $< 0.01$ \\ 
  Quick A-2 Rabin & CODE & $512$ & $369.5$ & $2.3$ & $18.63$ & $< 0.01$ & $2.05$ & $< 0.01$ & $0.65$ & $< 0.01$ \\ 
  Quick A-3 Rabin & CODE & $512$ & $365.3$ & $3.7$ & $18.54$ & $< 0.01$ & $2$ & $< 0.01$ & $0.71$ & $< 0.01$ \\ 
  Quick HM-2 Rabin & CODE & $512$ & $344$ & $2.3$ & $20.21$ & $< 0.01$ & $2.05$ & $< 0.01$ & $0.75$ & $0.01$ \\ 
  Quick HM-3 Rabin & CODE & $512$ & $336.7$ & $4.1$ & $20.22$ & $< 0.01$ & $2.01$ & $< 0.01$ & $0.76$ & $< 0.01$ \\ 
  Rabin & RAND & $512$ & $208.8$ & $4.6$ & $34.11$ & $0.01$ & $2.19$ & $< 0.01$ & $0.15$ & $< 0.01$ \\ 
  Quick A-2 Rabin & RAND & $512$ & $354.3$ & $1.7$ & $18.76$ & $< 0.01$ & $2.03$ & $< 0.01$ & $0.57$ & $< 0.01$ \\ 
  Quick A-3 Rabin & RAND & $512$ & $299.6$ & $5.4$ & $18.81$ & $< 0.01$ & $1.75$ & $< 0.01$ & $0.9$ & $< 0.01$ \\ 
  Quick HM-2 Rabin & RAND & $512$ & $305$ & $3.4$ & $20.39$ & $< 0.01$ & $1.99$ & $< 0.01$ & $0.73$ & $< 0.01$ \\ 
  Quick HM-3 Rabin & RAND & $512$ & $240.8$ & $6.7$ & $21$ & $< 0.01$ & $1.54$ & $< 0.01$ & $1.24$ & $< 0.01$ \\ 
  Rabin & CODE & $8{,}192$ & $206.5$ & $3.1$ & $34.32$ & $0.01$ & $2.2$ & $< 0.01$ & $0.15$ & $< 0.01$ \\ 
  Quick A-2 Rabin & CODE & $8{,}192$ & $375.4$ & $3.1$ & $18.35$ & $< 0.01$ & $2.03$ & $< 0.01$ & $0.62$ & $< 0.01$ \\ 
  Quick A-3 Rabin & CODE & $8{,}192$ & $374.4$ & $4.6$ & $18.07$ & $< 0.01$ & $2.01$ & $< 0.01$ & $0.65$ & $< 0.01$ \\ 
  Quick HM-2 Rabin & CODE & $8{,}192$ & $374.2$ & $3.9$ & $18.47$ & $< 0.01$ & $2.02$ & $< 0.01$ & $0.64$ & $< 0.01$ \\ 
  Quick HM-3 Rabin & CODE & $8{,}192$ & $374.3$ & $2.3$ & $18.18$ & $< 0.01$ & $2.01$ & $< 0.01$ & $0.66$ & $< 0.01$ \\ 
  Rabin & RAND & $8{,}192$ & $205.5$ & $3.4$ & $34.31$ & $0.01$ & $2.19$ & $< 0.01$ & $0.15$ & $< 0.01$ \\ 
  Quick A-2 Rabin & RAND & $8{,}192$ & $373.8$ & $8.1$ & $17.55$ & $< 0.01$ & $2.03$ & $< 0.01$ & $0.62$ & $< 0.01$ \\ 
  Quick A-3 Rabin & RAND & $8{,}192$ & $371$ & $2.0$ & $17.57$ & $< 0.01$ & $2$ & $< 0.01$ & $0.62$ & $< 0.01$ \\ 
  Quick HM-2 Rabin & RAND & $8{,}192$ & $369.4$ & $5.6$ & $17.67$ & $< 0.01$ & $2.02$ & $< 0.01$ & $0.66$ & $< 0.01$ \\ 
  Quick HM-3 Rabin & RAND & $8{,}192$ & $354.6$ & $11.5$ & $17.73$ & $< 0.01$ & $2$ & $< 0.01$ & $0.64$ & $0.01$ \\ 
   \bottomrule
\end{tabular}


==> tables/acs.tex <==
\begin{table}[]
\begin{center}
\setlength\tabcolsep{3.8pt}
\footnotesize
\begin{tabularx}{\columnwidth}{lllllll}
\toprule
\multirow{2}{*}{\textbf{Data}} & %
\multirow{2}{*}{\textbf{Alg.}} & %
\multicolumn{5}{c}{\textbf{Target Chunk Sizes}} \\
& & \textbf{32\,kB} & \textbf{64\,kB} & \textbf{128\,kB} & \textbf{256\,kB} & \textbf{512\,kB} \\
\midrule

\multirow{5}{*}{TAR} & FSC & 32\,kB & 64\,kB & 128\,kB & 256\,kB & 511\,kB \\
         & Rabin & 31\,kB (-3\%)& 57\,kB (-12\%) & 105\,kB (-22\%) & 192\,kB (-33\%) & 354\,kB (-45\%) \\
         & Buzhash & - & - & - & 165\,kB (-55\%) & - \\
         & FastCDC & 45\,kB (+28\%) & 89\,kB (+28\%)	 & 177\,kB (+28\%) & 357\,kB (+28\%) & 708\,kB (+28\%) \\
         & AE & 36\,kB (+11\%) & 73\,kB (+12\%) & 147\,kB (+13\%) & 297\,kB (+14\%) & 599\,kB (+15\%) \\
\midrule
\multirow{5}{*}{WEB} & FSC & 32\,kB & 64\,kB & 128\,kB & 255\,kB & 509\,kB (-1\%) \\
         & Rabin & 33\,kB (+4\%)	 & 60\,kB (-8\%) & 109\,kB (-18\%) & 206\,kB (-25\%)	& 393\,kB (-30\%) \\
         & Buzhash & - & - & - & 189\,kB (-35\%) & - \\
         & FastCDC & 39\,kB (+18\%)	& 77\,kB (+17\%) & 154\,kB (+17\%)	 & 310\,kB (+17\%)	& 614\,kB (+17\%) \\
         & AE & 32\,kB (+1\%) & 64\,kB & 129\,kB (+1\%) & 256\,kB & 513\,kB \\
\midrule
\multirow{5}{*}{LNX} & FSC & 32\,kB & 64\,kB & 128\,kB & 256\,kB & 512\,kB \\
         & Rabin & 32\,kB & 64\,kB & 127\,kB (-1\%) & 250\,kB (-2\%) & 496\,kB (-3\%) \\
         & Buzhash & - & - & - & 245\,kB (-5\%) & - \\
         & FastCDC & 38\,kB (+15\%) & 75\,kB (+15\%) & 150\,kB (+15\%)	 & 300\,kB (+15\%) & 601\,kB (+15\%) \\
         & AE & 32\,kB (+1\%) & 64\,kB & 128\,kB & 256\,kB & 511\,kB \\
\midrule
\multirow{5}{*}{DLF} & FSC & 32\,kB & 64\,kB & 127\,kB (-1\%) & 252\,kB (-2\%) & 494\,kB (-4\%) \\
         & Rabin & 32\,kB & 64\,kB & 126\,kB (-2\%) & 245\,kB (-5\%) & 469\,kB (-9\%) \\
         & Buzhash & - & - & - & 239\,kB (-7\%) & - \\
         & FastCDC & 37\,kB (+15\%) & 75\,kB (+15\%)	 & 150\,kB (+15\%)	 & 299\,kB (+15\%) & 597\,kB (+14\%) \\
         & AE & 32\,kB & 64\,kB & 127\,kB (-1\%) & 251\,kB (-2\%) & 493\,kB (-4\%) \\
\midrule
\multirow{5}{*}{MOV} & FSC & 32\,kB & 64\,kB & 128\,kB & 256\,kB & 512\,kB \\
         & Rabin & 40\,kB (+21\%) & 80\,kB (+20\%) & 159\,kB (+19\%)	& 316\,kB (+19\%) & 619\,kB (+17\%) \\
         & Buzhash & - & - & - & 249\,kB (-3\%) & - \\
         & FastCDC & 36\,kB (+11\%) & 72\,kB (+11\%) & 143\,kB (+11\%) & 286\,kB (+11\%) & 572\,kB (+11\%) \\
         & AE & 32\,kB (-1\%) & 63\,kB (-1\%) & 126\,kB (-1\%) & 252\,kB (-1\%) & 505\,kB (-1\%) \\
\midrule

& & \textbf{256\,B} & \textbf{512\,B} & \textbf{1\,kB} & \textbf{2\,kB} & \textbf{4\,kB} \\
\midrule

\multirow{5}{*}{PNG} & FSC & 255\,B & 511\,B & 1023\,B & 2045\,B & 4085\,B \\
         & Rabin & 325\,B (+21\%) & 651\,B (+21\%) & 1303\,B (+21\%)	 & 2603\,B (+21\%) & 5\,kB (+21\%) \\
         & Buzhash & - & - & - & - & - \\
         & FastCDC & 299\,B (+14\%) & 598\,B (+14\%)	 & 1196\,B (+14\%) & 2392\,B (+14\%) & 5\,kB (+14\%) \\
         & AE & 340\,B (+25\%) & 657B (+22\%) & 1238\,B (+17\%) & 2307\,B (+11\%) & 4\,kB (+6\%) \\
\midrule
\multirow{5}{*}{JPEG} & FSC & 255\,B & 511\,B & 1021\,B & 2039\,B & 4063\,B (-1\%) \\
         & Rabin & 326\,B (+22\%) & 655\,B (+22\%) & 1307\,B (+22\%) & 2607\,B (+21\%) & 5\,kB (+21\%) \\
         & Buzhash & - & - & - & - & - \\
         & FastCDC & 300\,B (+15\%) & 600\,B (+15\%)	 & 1199\,B (+15\%)	 & 2393\,B (+14\%) & 5\,kB (+14\%) \\
         & AE & 330B (+23\%)	 & 633\,B (+19\%) & 	1195\,B (+14\%)	& 2256\,B (+9\%) & 4\,kB (+5\%) \\
\midrule
\multirow{5}{*}{PDF} & FSC & 255\,B & 511\,B & 1023\,B & 2047\,B & 4093\,B \\
         & Rabin & 309\,B (+17\%) & 618\,B (+17\%)	 & 1236\,B (+17\%) & 2459\,B (+17\%) & 5\,kB (+16\%) \\
         & Buzhash & - & - & - & - & - \\
         & FastCDC & 314\,B (+18\%) & 627\,B (+18\%)	 & 1259\,B (+19\%)	& 2527\,B (+19\%) & 5\,kB (+19\%) \\
         & AE & 318\,B (+20\%)	 & 623\,B (+18\%)	 & 1189\,B (+14\%) & 2298\,B (+11\%) & 4\,kB (+8\%) \\

\bottomrule
\end{tabularx}
\caption{Real average chunk sizes produced during our experiments on different datasets and their deviation from the target chunk sizes.}
\end{center}
\end{table}

==> tables/file-types.tex <==
\begin{tabularx}{0.72\textwidth}{lll}
\toprule
\textbf{Occurrences (\%)} & \textbf{MIME-Type} & \textbf{Charset} \\
\midrule
213,355 (78\%) & application/octet-stream & binary \\
27,025 (10\%) & application/json & us-ascii \\
9,624 (3.5\%) & image/png & binary \\
4,550 (1.7\%) & image/jpeg & binary \\
4,283 (1.6\%) & application/pdf & binary \\
3,413 (1.3\%) & text/plain & us-ascii \\
3,388 (1.2\%) & application/json & utf-8 \\
3,363 (1.2\%) & application/x-dosexec & binary \\
\bottomrule
\end{tabularx}

==> tables/quickcdc.tex <==
\begin{tabular}{|c|c|c|c|}
    \hline
     \textbf{Chunk ID} & \textbf{Front} & \textbf{End} & \textbf{Length} \\ \hline
     $i$ & \texttt{3F A2 7C} & \texttt{FF 41 8E} & 7984 \\ \hline
     $i+1$ & \texttt{12 55 9B} & \texttt{2A F7 0D} & 9830 \\ \hline
    $i+2$ & \texttt{8C 09 E4} & \texttt{71 2B 63} & 8601 \\ \hline
\end{tabular}

==> tables/speed-bench.tex <==
\begin{table}[h]
\begin{center}
\begin{tabularx}{0.9\textwidth}{lrrrr}
\toprule
\textbf{Algorithm} & \textbf{Speed} & \textbf{Processed} & \textbf{Alloc. Bytes} & \textbf{Mem. Alloc.} \\
\midrule
FSC & 37.53\,s/op & 2,793.71\,MB/s & 104.86\,MB/op & 405 allocs/op \\
Rabin & 610.60\,s/op & 171.73\,MB/s & 108.71\,MB/op & 968 allocs/op \\
Buzhash & 103.71\,s/op & 1,038.99\,MB/s & 106.54\,MB/op & 421 allocs/op \\
FastCDC & 66.48\,s/op & 1,577.21\,MB/s & 1.05\,MB/op & 3 allocs/op \\
AE & 249.19\,s/op & 420.80\,MB/s & 318.19\,MB/op & 802 allocs/op \\
\bottomrule
\end{tabularx}
\end{center}
\caption{Benchmark for speed and memory utilization of all chunking algorithms in comparison on a generated test file of 100MB and a target chunk size of 256\,kB. An operation (``op'') equals the process of splitting the test file into its chunks.}
\label{table:speedBench}
\end{table}
